Walk-Sums, Continued Fractions and Unique Factorisation on Digraphs

We show that the series of all walks between any two vertices of any (possibly weighted) directed graph $\mathcal{G}$ is given by a universal continued fraction of finite depth and breadth involving the simple paths and simple cycles of $\mathcal{G}$. A simple path is a walk forbidden to visit any vertex more than once. We obtain an explicit formula giving this continued fraction. Our results are based on an equivalent to the fundamental theorem of arithmetic: we demonstrate that arbitrary walks on $\mathcal{G}$ factorize uniquely into nesting products of simple paths and simple cycles, where nesting is a product operation between walks that we define. We show that the simple paths and simple cycles are the prime elements of the set of all walks on $\mathcal{G}$ equipped with the nesting product. We give an algorithm producing the prime factorization of individual walks, and obtain a recursive formula producing the prime factorization of sets of walks. Our results have already found applications in machine learning, matrix computations and quantum mechanics.

==> Complexity.tex <==
\section{Complexity of the prime factorisation}\label{StarHeightsection}
\sjt{In this last section we present results} concerning the computational complexity of the prime factorisation of walks.

The algorithm for factoring individual walks provided in \S\ref{Algosection} is easily shown to be efficient, with a time complexity for the worst case scenario scaling quadratically with the walk length. \sjt{Conversely, we note that since the primes (i.e.~the simple cycles and simple paths of $\G$)} are difficult to identify, we expect the factorised form of the set of \textit{all} walks $W_{\G;\alpha\omega}$ to be difficult to construct. For example, if \sjt{$\G$ is Hamiltonian,} the Hamiltonian cycle or path must appear in the factorisation of at least one walk set. Consequently, we expect that factoring walk sets requires determining the existence of such a cycle or path, a problem which is known to be NP-complete \sjt{reference?}.

In order to formalise this observation, we now determine the star-height of the prime factorisation, as given by Theorem \ref{FactorBasis}, of any set $W_{\G;\,\alpha\omega}$. The star-height $h(\mathfrak{E})$ of a regular expression $\mathfrak{E}$ was introduced by Eggan \cite{Eggan1963} as the \sjt{depth of the most deeply-nested Kleene star in $\mathfrak{E}$.} This quantity characterises the structural complexity of formal expressions. \sjt{As Example \ref{exampleK3} illustrates, the prime factorisations of sets of walks typically have a non-zero star-height (see e.g.~\eqref{W11K3Factor}).} Furthermore, the proofs of Theorems \ref{FactorSum} and \ref{FactorSumOfWeights} show that the star-height of $W_{\G;\,\alpha\omega}$ is equal to the depth of the continued fraction generated by Theorems \ref{FactorSum} and \ref{FactorSumOfWeights}. In this section we obtain an exact recursive expression for $h(W_{\G;\,\alpha\omega})$. The following result says that the problem of  evaluating $h(W_{\G;\,\alpha\omega})$ is nonetheless NP-complete on undirected connected graphs :

\begin{theorem}\label{StarHeighGraph}
Let $\G$ be a finite undirected connected graph, possibly with self-loops. Let $\alpha$ and $\omega$ be two vertices on it. We define $\mathrm{L}\Pi_{\G;\,\alpha}$ to be \sjt{\textbf{the set of longest simple paths starting at $\alpha$,}} with $\ell_\alpha$ their length.
Then
\begin{equation}
h\big(W_{\G;\,\alpha\omega}\big)=h\big(W_{\G;\,\alpha\alpha}\big)=\begin{cases}\ell_\alpha+1,&\text{if there exists $p\in \mathrm{L}\Pi_{\G;\,\alpha}$ such that the}\\
&\text{last vertex of $p$ sustains a self loop},\\\ell_\alpha,&\textrm{otherwise}.\end{cases}
 \end{equation}
The problem of determining $h(W_{\G;\,\alpha\omega})$ and $h(W_{\G;\,\alpha\alpha})$ is equivalent to determining the existence of a Hamiltonian path starting at $\alpha$. It is therefore NP-complete.
\end{theorem}

%In \S \ref{StarHeightProof} we obtain an exact recursive expression for $h(W_{\G;\,\alpha\omega})$ with $\G$ an arbitrary digraph and demonstrate Theorem \ref{StarHeighGraph}.
\sjt{To prove the Theorem, we begin} by establishing an exact recursive relation yielding the star-height of the prime factorisation of a walk-set. This relation will be necessary to prove Theorem \ref{StarHeighGraph}.
\vspace{1.5mm}\begin{lemma}[Star-height]\label{StarHeight} Let $(\mu_c,\nu_0,\nu_p)\in \mc{V}(\G)^3$. \sjt{Then the star-height of the factorised expression for the set of cycles $W_{\G;\,\mu_c\mu_c}$, denoted by $h\big(W_{\G;\,\mu_c\mu_c}\big)$, is given by the recursive relation
\begin{align}\label{hCycles}
  h\big(W_{\G;\,\mu_c\mu_c}\big) = \begin{cases}0 & \text{if $\,\Gamma_{\G;\,\mu_c}=\emptyset$},
  \\ 1+\underset{\Gamma_{\G;\,\mu_c}}{\max} \:\underset{1 \le i \le c-1}{\max}\:\: h\big(W_{\G\backslash\{\mu_c,\,\mu_1,\cdots,\,\mu_{i-1}\};\,\mu_i\mu_i}\big)
  &\text{otherwise}, \\ \end{cases}
 \end{align}
 where the first maximization in the second line runs over all simple cycles $\mu_c \mu_1\cdots \mu_{c-1} \mu_c\in \Gamma_{\G;\,\mu_c}$.} The star-height $h\big(W_{\G;\,\nu_0\nu_p}\big)$ of the factorised expression for the set of open walks $W_{\G;\,\nu_0\nu_p}$ is
\begin{equation}\label{hOpen}
  h\big(W_{\G;\,\nu_0\nu_p}\big) = \underset{\Pi_{\G;\,\nu_0\nu_p}}{\max} \:\underset{0 \le i \le p}{\max}\:\: h\big(W_{\G\backslash\{\nu_0,\nu_1,\cdots,\nu_{i-1}\};\,\nu_i\nu_i}\big),
\end{equation}
where $(\nu_0 \nu_1\cdots \nu_{p-1}\nu_p)\in \Pi_{\G;\,\nu_0\nu_p}$.
\end{lemma}
\begin{proof}
These results follow from Eqs.~(\ref{WG}, \ref{AG}).
We have $W_{\G;\,\mu_c\mu_c}=A^\ast_{\G;\,\mu_c}$
\sjt{and thus if $A_{\G;\,\mu_c}=\Gamma_{\G;\,\mu_c}=\emptyset$ is empty, then $W_{\G;\,\mu_c\mu_c} = \{(\mu_c)\}$ and $h(W_{\G;\,\mu_c\mu_c})=0$.} Otherwise,
$h(W_{\G;\,\mu_c\mu_c})=1+h(A_{\G;\,\mu_c})$. Now by Eq.~(\ref{AG}) we have \vspace{-1mm}
\begin{equation}
\vspace{-1mm}h\big(A_{\G;\,\mu_c}\big)=\underset{\Gamma_{\G;\,\mu_c}}{\max} \:\underset{1 \le i \le c-1}{\max}\:\: h\big(A_{\G\backslash\{\mu_c,\,\mu_1,\cdots,\,\mu_{i-1}\};\,\mu_i\mu_i}\big),
\end{equation}
and since $W_{\G\backslash\{\mu_c,\,\mu_1,\cdots,\,\mu_{i-1}\};\,\mu_i\mu_i}=
A^\ast_{\G\backslash\{\mu_c,\,\mu_1,\cdots,\,\mu_{i-1}\};\,\mu_i\mu_i}$, Eq.~(\ref{hCycles}) follows. By similar reasoning, Eq.~(\ref{hOpen}) is obtained from Eq.~(\ref{WG}); we omit the details.\qed
\end{proof}
%
%\begin{remark}[Cycle rank]
%The cycle rank $r(\G)$ of a graph $\G$ \cite{Eggan1963} quantifies the minimum number of vertices that must be removed from $\G$ in order for its largest strongly connected component to be acyclic.
%Contrary to what one might expect, the star-heights $h(W_{\G;\,\nu_0\nu_p})$ and $h(W_{\G;\,\mu_c\mu_c})$ are not equal to the cycle rank $r(\G)$. This is because of an essential difference between Proposition \ref{StarHeight} and the definition of $r(\G)$: when calculating the star-height of a prime factorisation, the removal of vertices takes place along simple paths and simple cycles of $\G$. Conversely, the definition of $r(\G)$ allows the removal of non-neighbouring vertices throughout the graph. By this argument we see that the cycle rank is only a lower bound on the star-height of factorised forms of walk sets: $h(W_{\G;\,\nu_0\nu_p})\geq r(\G)$ and $h(W_{\G;\,\mu_c\mu_c})\geq r(\G)$.
%\end{remark}

%We note that nested Kleene stars appear whenever one can nest at least one non-trivial simple cycle off an internal vertex of another simple cycle. Thus, we expect the star-height to equal the length of the longest chain of recursively nested non-trivial simple cycles on $\G$.

\vspace{1.5mm}\noindent We are now ready to prove Theorem \ref{StarHeighGraph}.
\begin{proof}
We begin by proving the result for $h(W_{\G;\,\alpha\alpha})$.
Let $p_\alpha=(\alpha\nu_2\cdots\nu_{\ell_\alpha})\in\mathrm{L}\Pi_{\G;\,\alpha}$. Consider the cycle $w_\alpha$ off $\alpha$ produced by traversing $p_\alpha$ from start to finish, then traversing the loop $(\nu_{\ell_\alpha}\nu_{\ell_\alpha})$ if it exists, then returning to $\alpha$ along $p_\alpha$.
The proof consists of showing that $w_\alpha$ comprises the longest possible chain of recursively nested simple cycles on $\G$.

To this end, consider the factorisation of $w_\alpha$. Let $L_\alpha$ be equal to $(\nu_{\ell_\alpha}\nu_{\ell_\alpha})$, if this loop exists, or $(\nu_{\ell_\alpha})$, otherwise. Then observe that \sjt{$w_\alpha$ can be written as}
\begin{equation}\label{waFactor}
w_\alpha= b_0\odot \Big(b_1\odot\cdots\odot \big(b_{\ell_\alpha-1}\odot (b_{\ell_\alpha}\odot L_\alpha)\big)...\Big)\,,
\end{equation}
where $b_{0\leq j\leq \ell_\alpha-1}$ is the back-track $b_j=(\nu_{j}\nu_{j+1}\nu_j)\in \Gamma_{\G\backslash\{\alpha,\nu_2\cdots\nu_{j-1}\};\,\nu_j}$, \sjt{and} we have identified $\alpha$ with $\nu_0$ for convenience. Equation (\ref{waFactor}) shows that $w_\alpha$ is a chain of $\ell_\alpha$ (or $\ell_\alpha+1$, if the loop $(\nu_{\ell_\alpha}\nu_{\ell_\alpha})$ exists) recursively nested non-trivial simple cycles, and $W_{\G;\,\alpha\alpha}$ must involve at least this many nested Kleene stars.

To see that this chain is the longest, suppose that there exists a walk $w'$ involving $n>\ell_\alpha$ \big(or $n>\ell_\alpha+1$, if the loop $(\nu_{\ell_\alpha}\nu_{\ell_\alpha})$ exists\big) non-trivial recursively nested simple cycles $c_1,\cdots,\, c_n$; that is, $c_1\odot\big(\cdots \odot(c_{n-1}\odot c_n)\big)\subseteq w'$. Then, by the nestable property, the vertex sequence $s\subseteq w'$ joining the first vertex of $c_1$ to the last internal vertex of $c_n$ defines a simple path $p'$ of length $\ell(p')\geq n>\ell_\alpha$. This is in contradiction to the definition of $\ell_\alpha$, and thus $w'$ does not exist.
Consequently, $h(W_{\G;\,\alpha\alpha})= \ell_\alpha+1$ if the loop $(\nu_{\ell_\alpha}\nu_{\ell_\alpha})$ exists, or $\ell_\alpha$, if there is no self-loop on $\nu_{\ell_\alpha}$.



We now turn to determining $h(W_{\G;\,\alpha\omega})$. Combining Eq.~(\ref{hOpen}) with the result for $h(W_{\G;\,\alpha\alpha})$ obtained above yields
\begin{equation}\label{eq:hstepdemo}
h\big(W_{\G;\,\alpha\omega}\big)= \underset{\Pi_{\G;\,\nu_0\nu_p}}{\max} \:\underset{0 \le i \le p}{\max}\:\:\begin{cases}
\ell_{\nu_i}\big(\G\backslash\{\alpha,\ldots,\nu_{i-1}\}\big)+1&\text{if there is a self-loop on vertex }\nu_{i},\\
\ell_{\nu_i}\big(\G\backslash\{\alpha,\ldots,\nu_{i-1}\}\big)&\mathrm{otherwise},
\end{cases}
\end{equation}
where $\ell_{\nu_i}(\G\backslash\{\alpha,\ldots,\nu_{i-1}\})$ is the length of the longest simple path $p_{\nu_i}$ off vertex $\nu_i$ on $\G\backslash\{\alpha,\ldots,\nu_{i-1}\}$, and $\nu_{\ell_{\nu_i}}$ is the last vertex of $p_{\nu_i}$. Finally, we note that $p_\alpha$ is the longest of all the simple paths $p_{\nu_i}$: since $\G$ is undirected and connected, it is strongly connected, and since $\G\backslash\{\alpha,\ldots,\nu_{i-1}\}$ is a subgraph of $\G$ strictly smaller than $\G$, then $p_{\nu_i}$ must be shorter than $p_{\alpha}$. Therefore Eq.~(\ref{eq:hstepdemo}) yields $h(W_{\G;\,\alpha\omega})= h(W_{\G;\,\alpha\alpha})$.

It follows from these results that in order to determine the star-height of the factorised form of any walk set on an \sjt{undirected connected graph $\G$,} one must determine the existence of a Hamiltonian path on $\G$. Consequently, the problem of determining $h\big(W_{\G;\,\alpha\omega}\big)$ and $h\big(W_{\G;\,\alpha\alpha}\big)$ is NP-complete.\qed
\end{proof}

Theorem \ref{StarHeighGraph} means that just determining the complexity of prime factorisations on ordinary graphs is already quite hard. This result may be considered unsurprising in view of the fact that prime factorisations are known to be difficult to obtain, e.g. in the case of integers. Here, however, the origin of the difficulty is different from that in the case of integer factorisation: it resides in factoring \emph{all} the sets of \emph{all} the walks between any two vertices of a connected graph or in computing the star-heights of the factorised forms.
%At the opposite, factoring an individual walk using Algorithm \ref{AlgoCanFac} is surprisingly easy: we can show that the time complexity of the algorithm scales quadratically with the length $\ell(w)$ of the walk $w$ being factorised in the worst case scenario, and only linearly with $\ell(w)$ in the typical case scenario. 

==> Factorization.tex <==
\section{Prime Factorisation on Digraphs}\label{sec:WalkFactor}
In this section, we prove the existence and uniqueness of the factorisation of individual walks on digraphs into nesting products of prime walks, which we identify to be the simple paths and simple cycles. We provide an algorithm \sjt{that factors} walks.
Second, we give an explicit formula expressing the set of all walks between any two vertices of any digraph \sjt{as a collection of nested sets} of prime walks. \sjt{We will use this result in the next section} to obtain representations for the series of all walks on any digraph which involve only prime walks. For each result we present, we provide a simple example demonstrating its use.

\subsection{Existence and uniqueness of the prime factorisation of walks}\label{FTAdigraph}
The fundamental theorem of arithmetic is arguably the most important \sjt{result in number theory} \cite{Hardy1979}. It establishes the central role \sjt{played by the prime numbers, and has many profound consequences on} the properties of integers. We now present its analogue for individual walks on arbitrary digraphs.

We begin by presenting the notion \sjt{of a factorisation of a walk and stating the conditions under which two factorisations are equivalent.}
%
%\begin{definition}[Factorisation of a walk]
\sjt{A factorisation of a walk $w$ on $\G$, denoted $\mathsf{Fac}\,w$, is a decomposition of $w$ into a nesting product of other walks on $\G$, which we term the factors of $w$. Recombining the factors of $w$ with the nesting operation reproduces the original walk $w$.} Since nesting is neither commutative nor associative, it is necessary to be cautious about equivalent factorisations of a walk. We say that two factorisations $\mathsf{Fac}\,w$ and $\mathsf{Fac}'\,w$ of a walk $w$ are equivalent, denoted $\mathsf{Fac}\,w\equiv \mathsf{Fac}'\,w$, if and only if one can be obtained from the other through the reordering of parentheses and factors, and up to nesting with trivial walks, without modifying $w$. In particular, equivalent factorisations of a walk are made up of the same non-trivial factors. Equivalent factorisations are generated by the following operations:
\begin{itemize}
\vspace{-1mm}
\item[i)] Multiplication by trivial factors (i.e. trivial walks).
\item[ii)] Let $w, a$ and $b$ be walks such that $(w,a)$ and $(w,b)$ are nestable. Then one can replace $(w\odot a)\odot b$ by $(w\odot b)\odot a$ if and only if $a$ and $b$ do not have any vertex in common.
\item[iii)] Let $w, a$ and $b$ be walks such that $(w,a)$ and $(a,b)$ are nestable but $(w,b)$ is \emph{not} nestable. Then one can replace $(w\odot a)\odot b$ by $w\odot (a \odot b)$.
\end{itemize}
\vspace{-1mm}From now on, we shall speak of walk factorisations up to equivalence, that is up to the application \sjt{of one or more} of the above operations.

%\end{definition}
%\noindent As an example illustrating factorisations, consider the walk $w=(1323312)$. Then $\mathfrak{f}_1(w)=12\odot 132331$ is a factorisation of $w$. Another factorisation of this walk is $\mathfrak{f}_2(w)=12\odot (131\odot 3233)$.

%\begin{definition}[Equivalent factorisations]\label{eqFacDef}
%Let $w$ be a walk on $\G$ and $\mathfrak{f}_1(w)$ a factorisation of it.
%
%\end{definition}

%\noindent $\blacktriangleright$ Two factorisations that do not have the same set of factors are non-equivalent.

\vspace{2mm}Of particular interest is the factorisation of a walk into nesting products of prime walks. Following standard definitions \cite{Lang2002,Lam2001}, a walk $w$ is said to be \textit{prime} with respect to nesting if and only if for all nestable couples of walks $(w',w'')$ such that $w\,|\,w'\odot w''$ then $w\,|\,w'$ or $w\,|\,w''$. It is a central result of this article that the prime factorisation of any walk $w$ exists and is unique and the set of primes factors of $w$ is uniquely determined by $w$:

\begin{theorem}[Prime factorisation of walks]\label{FundamentalthmDigraph}
Any walk on $\G$ factorises uniquely into nesting products \sjt{of prime walks:} the simple paths and simple cycles on $\G$.
%Then $K\G_\odot$ is a noncommutative nonassociative unique factorisation near-algebra with zero-divisors.
\end{theorem}
%\vspace{-2mm}\noindent $\blacktriangleright$ Theorem \ref{FundamentalthmDigraph} is proven in \S \ref{ExistsProof}.
The theorem makes three statements concerning the prime factorisation of a walk: i) it always exists; ii) it is unique; and iii) a walk is prime if and only if it is a simple path or a simple cycle.

%From now on we shall thus speak of \emph{the} prime factorisation $\mc{F}_{\odot}(w)$ of a walk $w$. Below we give an algorithm that produces $\mc{F}_{\odot}(w)$ for an arbitrary walk.

%Later on, we will use the same algorithm to obtain a general formula giving the prime factorisation of walk sets into nesting products of prime walk sets.

\vspace{2mm}The proof of Theorem \ref{FundamentalthmDigraph} is organized as follows. We begin by showing that a walk is \sjt{irreducible -- that is, that it cannot be expressed as a nesting product of two or more non-trivial walks -- if and only if} it is a simple path or a simple cycle. Second, we show that the factorisation of a walk into nesting products of irreducible walks always exists and is unique. Third, we prove that a walk is prime if and only if it is a simple path or a simple cycle. \sjt{Taken together, these steps} establish Theorem \ref{FundamentalthmDigraph} as an equivalent to the fundamental theorem of arithmetic.\\


\textit{Proof }
Following standard definitions \cite{Lang2002,Lam2001}, a walk $w$ is \textit{irreducible} if, whenever there exists a divisor $w'$ of $w$, then either $w'$ is trivial, or $w'=w$ up to nesting with trivial walks (i.e. local identities). \sjt{A walk that is not irreducible is said to be \textit{reducible}. Then we have the following result:}

\begin{lemma}\label{irreducible}
A walk $w$ is irreducible if and only if it is a simple path or a simple cycle.
\end{lemma}
\begin{proof}
The forward direction is straightforward since simple paths and simple cycles have no repeated internal vertices.
For the backward direction, consider an irreducible walk $w$ and suppose that $w$ is neither a simple path nor a simple cycle. In this case, there exists an earliest vertex $\mu$ visited at least twice by $w$ (if $w$ is a cycle, then consider the earliest internal vertex visited at least twice by $w$). Now let $s_\mu\subset w$ be the vertex sequence joining the first appearance of $\mu$ to its final appearance in $w$, and let $w_\mu$ be the vertex sequence obtained from $w$ by replacing $s_\mu$ by $(\mu)$ in $w$. Then $(w_\mu,s_\mu)$ is a nestable couple of non-trivial walks and $w=w_\mu\odot s_\mu$, which is a contradiction.\qed
\end{proof}
%\begin{remark}[Identifying the simple paths and simple cycles]
%The simple paths and simple cycles of the digraph $\G$ can be systematically obtained via the powers of its nilpotent adjacency matrix  \cite{Staples2008,Schott2012}. The nilpotent adjacency matrix $\bar{\matr{A}}_\G$ is constructed by weighting the adjacency matrix $\matr{A}$ of $\G$ with formal variables $\zeta_{e}$, one for each directed edge $e$ and such that: i) $[\zeta_e,\zeta_{e'}]=0$ for any two edges $(e,e')\in\mc{E}(\G)$; and ii) $\zeta_e^2=0$ for all edges $e\in\mc{E}(\G)$. From this last property, it follows that only the simple paths and simple cycles a non-zero coefficient in powers of $\bar{A}_\G$.
%%\end{remark}
%We defer the proof of Proposition \ref{irreducible}, which requires intermediary results, to the next section \S \ref{ExistsProof}. Having established the definition and properties of the nesting product as well as the irreducible and prime elements it induces in $(W_\G,\,\odot)$, we turn to the factorisation of individual walks and walk sets.

%We obtain Lemma \ref{Factorisation} in two parts.
%Firstly, we give an algorithm that factorises an arbitrary walk into irreducible walks. This demonstrates existence of the factorisation. In a second part we show that any two factorisations of $w$ are equivalent.
%\vspace{1.5mm}


\begin{lemma}\label{factirred}
Any walk on $\G$ factorises uniquely into \sjt{nesting products of irreducible} walks.
\end{lemma}

\begin{proof}
We prove the lemma by induction on the walk length. Let $\mathcal{P}(n)$ be the following proposition: \textit{for any walk $w$ of length $\ell(w)\leq n$, there exists a unique factorisation of $w$ into nesting products of irreducible walks, denoted $\mathsf{Fac}_I\,w$.}\\
%, i.e. $\exists !\, \mathsf{Fac}\,w\in \mathcal{F}_w/\hspace{-.5mm}\equiv$.}

\noindent\textit{Base case:} we establish $\mathcal{P}(1)$. Consider a walk $w$ of length $\ell(w)=1$. Then $w$ is either a self-loop $(\alpha\alpha)$ or an edge $(\alpha\omega)$, for some vertices $\alpha$ and $\omega$. \sjt{In either case} it is irreducible. Furthermore, the factorised form of $w$ is $w$ itself and is clearly unique, so $\mathcal{P}(1)$ holds.\\

\vspace{-1mm}\noindent\textit{Induction:} \sjt{we show that for any $n \ge 1$, the ensemble of statements $\mathcal{P}(1),\mathcal{P}(2),\ldots,\mathcal{P}(n)$ imply $\mathcal{P}(n+1)$.} To this end, consider a walk $w$ of length $\ell(w)=n+1$. If $w$ is irreducible, then its \sjt{factorisation exists and is unique: this factorisation is $w$ itself, $\mathsf{Fac}_I\,w\equiv w$.}

In the case where $w$ is reducible, we begin by proving that \sjt{it has at least} one factorisation into products of irreducible walks. If $w$ is reducible, then there exists a nestable couple $(a,b)$ of non-trivial walks such that $w=a\odot b$. Necessarily $1\leq\ell(a),\,\ell(b)\leq n$ \sjt{and so by the induction hypothesis there exist unique factorisations of $a$ and $b$} into products of irreducible walks, $\mathsf{Fac}_I\,a$ and $\mathsf{Fac}_I\,b$. Then $\mathsf{Fac}_I\,w:=\mathsf{Fac}_I\,a\odot \mathsf{Fac}_I\,b$ is a valid factorisation of $w$ into irreducible walks.

Now suppose that there exists a second factorisation $\mathsf{Fac}'_I\,w$ of $w$ into irreducibles, which is \sjt{different from the first:} $\mathsf{Fac}_I\,w\nequiv \mathsf{Fac}_I'\,w$. Since $\mathsf{Fac}_I'\,w$ exists, there exists a nestable couple $(c,d)$ of non-trivial \sjt{walks such that $w=c\odot d$, $1\leq\ell(c)\le n$, $1 \le \ell(d)\leq n$, and $\mathsf{Fac}_I'\,w=\mathsf{Fac}_I\,c\odot \mathsf{Fac}_I\,d$.}

\sjt{Consider the case where $a=c$ and $b=d$. Then since $a$ and $b$ have length not greater than $n$, it follows from the induction hypothesis that the factorisation of $a$ into products of irreducible walks exists and is unique. Thus $a=c$ implies that $a$ and $c$ have the same factorisation into irreducible walks: $\mathsf{Fac}_I\,a\equiv \mathsf{Fac}_I\,c$. By analogous reasoning, $b=d$ implies that $\mathsf{Fac}_I\,b\equiv \mathsf{Fac}_I\,d$. In this situation $\mathsf{Fac}_I\,w$ and $\mathsf{Fac}_I'\,w$ are equivalent and $\mathcal{P}(n+1)$ holds.}

Otherwise, consider the case where $(a,b)\neq (c,d)$. Since $w=a\odot b=c\odot d$, the position of the cycle $d$ in the vertex sequence of $w$ must fall into one of the following three cases:
\begin{itemize}
\item[i)] \sjt{\underline{$d$ is included in $a$: $d\subseteq a$}}. Let $e:=a\cap c$ be the vertex sequence common to $a$ and $c$ \sjt{(see schematic representation below).}
Since $(a,b)$ is nestable $(e,b)$ is nestable, and similarly $(c,d)$ nestable implies $(e,d)$ nestable. Additionally $c=e\odot b$ and $a=e\odot d$. It follows that $\mathsf{Fac}_I\,w=\mathsf{Fac}_I\,a\odot \mathsf{Fac}_I\,b=\big(\mathsf{Fac}_I\,e\odot \mathsf{Fac}_I\,d\big)\odot \mathsf{Fac}_I\,b$ and $\mathsf{Fac}_I'\,w=\mathsf{Fac}_I\,c\odot \mathsf{Fac}_I\,d=\big(\mathsf{Fac}_I\,e\odot \mathsf{Fac}_I\,b\big)\odot \mathsf{Fac}_I\,d$. \sjt{Now since each of $e$, $b$ and $d$ have} length less than or equal to $n$, by the induction hypothesis their factorisations into irreducible walks exist and are unique. Consequently $\mathsf{Fac}_I\,w$ and $\mathsf{Fac}_I'\,w$ are equivalent and $\mathcal{P}(n+1)$ holds.
\begin{figure}[h!]
\centering
\includegraphics[scale=.45]{Case1.eps}
\caption*{\small Schematic representation of the vertex sequence of $w$ in the case $d\subseteq a$.} \label{fig:case1}
\end{figure}

\item[ii)]\underline{$d$ is included in $b$, $d\subseteq b$}. We proceed similarly \sjt{to case i).} Let $e:=b\cap c$ be the vertex sequence common to $b$ and $c$. \sjt{By construction, $e$ is a cycle. The couple $(a,b)$ and therefore $(a,e)$ are nestable, while the fact that $(c,d)$ is nestable implies that $(e,d)$ is also nestable. Thus we have $b=e\odot d$ and $c=a\odot e$, while $\mathsf{Fac}_I\,w=\mathsf{Fac}_I\,a\odot \mathsf{Fac}_I\,b=\mathsf{Fac}_I\,a\odot \big(\mathsf{Fac}_I\,e\odot \mathsf{Fac}_I\,d\big)$ and $\mathsf{Fac}_I'\,w=\mathsf{Fac}_I\,c\odot \mathsf{Fac}_I\,d=\big(\mathsf{Fac}_I\,a\odot \mathsf{Fac}_I\,e\big)\odot \mathsf{Fac}_I\,d$. Now since each of $a$, $e$ and $d$ has length less than or equal to $n$, by the induction hypothesis their factorizations into irreducible walks exist and are unique.} Consequently $\mathsf{Fac}_I\,w$ and $\mathsf{Fac}_I'\,w$ are equivalent and $\mathcal{P}(n+1)$ holds.
\begin{figure}[h!]
\centering
\includegraphics[scale=.45]{Case2.eps}
\caption*{\small Case $d\subseteq b$.} \label{fig:case2}
\vspace{-4mm}
\end{figure}
\item[iii)]\underline{$d$ straddles $a$ and $b$}. This case is essentially different from \sjt{i) and ii), and it is necessary to} distinguish subcases. Given that $a\odot b\neq0$ and $c\odot d\neq0$ by assumption, $b$ and $d$ must \sjt{both be cycles. Let the head vertex of $b$ be $\beta$, and the head vertex of $d$ be $\delta$.} Since $d$ straddles over $a$ and $b$, then $\delta$ is visited by both $a$ and $b$, and $\beta$ is visited by both $c$ and $d$.
\begin{figure}[h!]
\centering
\includegraphics[scale=.45]{Case3.eps}
\caption*{\small Case $d$ straddles over $a$ and $b$.} \label{fig:case3}
\vspace{-4mm}
\end{figure}

We first examine the situation where $\beta$ and $\delta$ are \sjt{different vertices. Then two cases exist:}\\
\textit{1) $a$ is a cycle off $\beta$}. Then $c$ visits $\beta$ before $\delta$, but $\beta$ is also visited by $d$. Thus the couple $(c,d)$ is non-nestable, which is a contradiction.\\
\textit{2) $a$ is an open walk from $\alpha$ to $\beta$, or $\beta$ appears only as an internal vertex of $a$}. In either situation, $a$ visits $\delta$ before the final appearance of $\beta$, but $\delta$ is also visited by $b$. Then the couple $(a,b)$ is non-nestable, which is a contradiction.

Finally, it remains to consider the case where $\beta$ and $\delta$ are identical. Then the last appearance of $\beta$ in $c$ must be the last vertex of $b$ (since $a\odot b$ nests $b$ into $a$ off the final appearance of $\beta$). However, $d$ straddles $a$ and $b$, which implies that $c$ visits $\beta$ after the last vertex of $d$; and $d$ is not nested into $c$ off the last appearance of $\beta$, a contradiction.  \sjt{Therefore case iii) is impossible:}  $w=a\odot b=c\odot d$ cannot hold with $d$ straddling $a$ and $b$.

\vspace{1mm}The analysis of case iii) shows that the unique factorisation of walks is a direct consequence of the conditions imposed on nestable couples. \sjt{\textbf{These conditions bare cycles from being broken across their boundaries. Indeed, had $d$ been allowed to straddle $a$ and $b$, its irreducible factors would not necessarily have appeared in the factorizations of $a$ and $b$, in particular if $d$ itself was irreducible.}}
\end{itemize}

\vspace{1mm}\noindent We have demonstrated that $\mathcal{P}(1)$ is true, and upon supposing that $\mathcal{P}(j)$ holds for all $j\leq n$, we have shown that $\mathcal{P}(n+1)$ holds. Consequently $\mathcal{P}(n)$ \sjt{holds for all $n \ge 1$.} The factorisation of a walk into nesting products of irreducible walks thus always exists and is unique.\qed
\end{proof}

%\vspace{1.5mm}We now establish Proposition \ref{irreducible} in two steps. First we determine the irreducible walks and then the prime walks.
%
%\begin{proposition}\label{IrreducibleProof}
%Let $w\in W_{\G}$. Then $w$ is irreducible if and only if $w$ is a simple path or a simple cycle.
%\end{proposition}

We complete the proof of Theorem \ref{FundamentalthmDigraph} by establishing that simple paths and simple cycles are prime:
\begin{lemma}\label{PrimeProof}
Let $w$ be a walk. Then $w$ is prime \sjt{if and only if it is} a simple path or a simple cycle.
\end{lemma}
\begin{proof}
Firstly, we prove the backward direction: \sjt{that if $w$ is a simple path or a simple cycle, then $w$ is prime.} Consider a walk $w$ and a nestable couple $(w_1,w_2)$ such that $w\,|\,w_1\odot w_2$. Since $w$ \sjt{is either a simple path or a simple cycle,} then, by Lemma \ref{irreducible}, $w$ is an irreducible factor appearing in the factorisation $\mathsf{Fac}_I\,(a\odot b)$ of $a\odot b$ into nesting products of irreducible walks. By uniqueness of this factorisation, Lemma \ref{factirred}, $w$ must either be an irreducible factor of $\mathsf{Fac}_I\,a$, implying $w\,|\,a$; or an irreducible factor of $\mathsf{Fac}_I\,b$, implying $w\,|\,b$; or both. It follows that $w$ is prime.
Secondly, we prove the forward direction: $w$ prime $\Rightarrow w$ is a simple path or a simple cycle. Suppose that there exists a prime walk $w$ which is neither a simple path nor a simple cycle. Then by, Lemma \ref{irreducible}, $w$ is reducible and there exists at least one nestable couple $(w_1,w_2)$ of non-trivial walks such that $w=w_1\odot w_2$. Clearly $w\,|\, w_1\odot w_2$, and $w_1$ and $w_2$ are strictly shorter than $w$. Therefore $w$ divides neither $w_1$ nor $w_2$, which is a contradiction.\qed
\end{proof}

\noindent \sjt{Taken together,} Lemmas \ref{irreducible}, \ref{factirred} and \ref{PrimeProof} establish Theorem \ref{FundamentalthmDigraph}.\qed

%\vspace{3mm}\noindent\textbf{}~\\
\subsection{An algorithm to factorise individual walks}\label{Algosection}
\sjt{Let $w$ be a walk on a digraph $\G$, and $S_{\!R}\big(\mathsf{Fac}_I\,w\big)$ be the set of \emph{reducible} factors appearing in a factorisation $\mathsf{Fac}_I\,w$ of $w$; that is
\begin{equation*}
  S_{\!R}\big(\mathsf{Fac}_I\,w\big) = \big\{ w' : w' \in \mathsf{Fac}_I\,w \text{ and $w'$ is reducible}  \big\}.
\end{equation*}
Algorithm} \ref{AlgoCanFac}, presented on p. \pageref{AlgoCanFac}, \sjt{then proceeds as follows. We begin by setting $\mathsf{Fac}\,w:=w$. Then an arbitrary reducible factor $a$ of $\mathsf{Fac}\,w$ is chosen and factorized into a nesting product of strictly shorter walks, yielding a factorization $\mathsf{Fac}\,a$. Next, $\mathsf{Fac}\,w$ is updated by replacing $a$ by its factorization $\mathsf{Fac}\,a$, an operation which we denote $\mathsf{Fac}\,w\rightarrow \mathsf{Fac}\,w\,/\,\{a\rightarrow \mathsf{Fac}\,a\}$. Finally, another reducible factor appearing in the updated factorisation $\mathsf{Fac}\,w$ is chosen, and the process is repeated. At each round, reducible factors are decomposed into nesting products of shorter walks. The algorithm stops when $S_{\!R}\big(\mathsf{Fac}\,w\big)$ is the empty set $\varnothing$, at which point $\mathsf{Fac}\,w$ is the prime factorisation of $w$.}

\setlength{\textfloatsep}{15pt}
\begin{algorithm}[t!]
%\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
%\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output\,}
\Input{A walk $w\in W_\G$}
\Output{The prime factorisation of $w$}
\BlankLine
$\mathsf{Fac}\,w:= w$\;
\vspace{1mm}
\While{$S_{\!R}\big(\mathsf{Fac}\,w\big)\neq\varnothing$}{
Choose any $a\in S_{\!R}\big(\mathsf{Fac}\,w\big)$\;
\vspace{1mm}
\eIf{$h(a)=t(a)=\mu$ and $a$ visits vertex $\mu$ a total of $k>2$ times}{
Let $c_{0},\cdots, c_{k}$ be the $k+1$ cycles off $\mu$ identified by splitting the vertex string of $a$ at each internal appearance of $\mu$.\\
\vspace{.5mm}
$\mathsf{Fac}\,w\rightarrow \mathsf{Fac}\,w\,/\,\{a\rightarrow(c_{0}\odot\cdots\odot c_{k})\}$\;
\hspace{5mm}\CommentSty{\% Replace $a$ with $(c_{0}\odot\cdots\odot c_{k})$ in $\mathsf{Fac}\,w$}\\}{
$w_0:=a$; $\mathsf{Fac}_0\,a:=w_0$\;
$j:=0$\;
\vspace{1mm}
\While{$w_j\notin \Pi_\G\cup \Gamma_\G$}{
Traverse $w_j$ from start to finish\\
\vspace{.5mm}
\eIf{$w_j$ is open}{Start the traversal on $h(w_j)$}{Start the traversal on the first internal vertex of $w_j$}
Upon arriving at the earliest vertex $\eta$ that $w_j$ visits at least twice, define :\\
\vspace{.5mm}
$s_{j+1}:=(\eta_{\textrm{first}}\cdots\eta_{\textrm{last}})$\;
\hspace{5mm}\CommentSty{\% Cycle from the first to the last occurrence of $\eta$ in $w_j$}\\
\vspace{.5mm}
$w_{j+1}:=w_j\,/\,\{s_{j+1}\rightarrow(\eta)\}$\;
\hspace{5mm}\CommentSty{\% Replace $s_{j+1}$ with $(\eta)$ in $w_j$}\\
\vspace{.5mm}
$\mathsf{Fac}_{j+1}\,a:=\mathsf{Fac}_{j}\,a\,/\,\{w_j\rightarrow(w_{j+1}\odot s_{j+1})\}$\;
\hspace{5mm}\CommentSty{\% Replace $w_{j}$ with $w_{j+1}\odot s_{j+1}$ in $\mathsf{Fac}_j\,a$}\\
\vspace{.5mm}
$j= j+1$\;
}
Let $m:=j$ and $r:=w_{m}\in \Pi_\G\cup \Gamma_\G$. Observe that $\mathsf{Fac}_m\,a=\Big(~\big((r\odot s_{m})\odot s_{m-1}\big)\odot\cdots\Big)\odot s_1$.\\
$\mathsf{Fac}\,w\rightarrow \mathsf{Fac}\,w\,/\,\{a\rightarrow \mathsf{Fac}_m\,a\}$\;
\hspace{5mm}\CommentSty{\% Replace $a$ with $\mathsf{Fac}_m\,a$ in $\mathsf{Fac}\,w$}
}
}
\vspace{.5mm}Prime factorisation of $w$ $\equiv \mathsf{Fac}\,w$\;
\hspace{5mm}\CommentSty{\% All the factors appearing in $\mathsf{Fac}\,w$ are now prime}
\caption{\mystrut{16pt}Prime factorisation of individual walks}\label{AlgoCanFac}
\end{algorithm}

\begin{proof}
\sjt{We first verify the correctness of the factorisations that Algorithm \ref{AlgoCanFac} performs, and second show that for any finite-length walk, the algorithm terminates and yields the prime factorisation.}

\sjt{\textbf{Initialization:} let $\mathsf{Fac}\,w$ be any factorisation of a walk $w$ on $\G$ of finite length $\ell(w)$ and let $a\in S_{\!R}\big(\mathsf{Fac}\,w\big)$.}

\textbf{If} $a$ is a cycle off $\mu$, and $\mu$ appears $k>0$ times \sjt{as an internal} vertex of $a$, then the algorithm splits the vertex string of $a$ at each internal appearance of $\mu$, thus producing $k+1$ \sjt{cycles $c_0, c_1,\ldots, c_k$ off $\mu$. Then by construction, $a=c_{0}\conc\cdots\conc c_{k}$, where $\conc$ is the concatenation operator.} Since nesting coincides with concatenation over the cycles, we have $c_{j}\conc\,c_{j+1}=c_{j}\odot c_{j+1}$ and
\begin{equation}\label{cycleSPLIT}
a=c_{0}\odot\cdots\odot c_{k},
\end{equation}
as claimed in the algorithm. Note that \sjt{each of the cycles $c_j$ is strictly shorter than $a$ and, by construction, does not have $\mu$ as an internal vertex.}

\textbf{Else}, let $(\alpha_1\,\alpha_2\cdots \alpha_n)$ be the vertex sequence of $a$. \sjt{Let $\eta$ be the earliest vertex that $a$ visits at least twice (or the earliest internal vertex, if $a$ is a cycle). Let $i$ and $f$ be the indices of the earliest and latest occurrences of $\eta$ in $a$, so that $\alpha_i=\alpha_f=\eta$, and set $s_{1}$ be the string of vertices $\eta_i\eta_{i+1}\cdots\eta_f$. Let $w_1$ be the walk obtained from $a$ by replacing $s_1$ by $\eta$. Then the couple $(w_1,\,s_{1})$ is nestable, since all vertices \sjt{$\alpha_{k}$ (where $k < i$)} are visited precisely once by $w$ and therefore cannot be visited by $s_{1}$. Then, by construction of $s_{1}$ and $w_1$, we have $\mathsf{Fac}_1\,a=w_1\odot s_{1}$.
By applying the same \sjt{reasoning} for the earliest vertex $\lambda$ visited at least twice by $w_1$ (the earliest internal vertex, if $w_1$ is a cycle), we construct a nestable couple $(w_2,\,s_2)$ with $w_1=w_{2}\odot s_{2}$ and thus $\mathsf{Fac}_2\,a=(w_{2}\odot s_{2})\odot s_{1}$. Proceeding similarly with $w_2$ and all the subsequent non-irreducible walks $w_j$ thus yields}
\begin{equation}\label{eq:FactorW}
\mathsf{Fac}_m\,a=\Big(~\big((r\odot s_{m})\odot s_{m-1}\big)\odot\cdots\Big)\odot s_1,
\end{equation}
\sjt{\textbf{where and $r\equiv w_m$ is irreducible, as claimed in the algorithm.[??]}}

\sjt{In either of the two cases above, $a$ is} factorised into nesting products of strictly shorter \sjt{walks which are either irreducible, or will in turn be factorised into nesting products of strictly shorter walks in a later step. After at most $\ell(w) - 1$ recursive factorizations, where $\ell(w)$ is the length of the original walk $w$,} all factors obtained are either irreducible or of length $1$. Since all walks of length 1 are irreducible, it follows that the algorithm factors \sjt{any walk of finite length into a nesting product of irreducible walks} in a finite number of steps. Finally, by Lemmas \ref{irreducible} and \ref{PrimeProof}, irreducible walks are \sjt{primes. The algorithm thus yields the prime factorisation of $w$.}\qed
\end{proof}

\begin{example}[The prime factorisation of a walk] In this example we give a detailed step-by-step example illustrating \sjt{the application of Algorithm} \ref{AlgoCanFac}.
Let $\G$ be the complete undirected graph on $4$ vertices with vertex labels \{1,2,3,4\}, and \sjt{consider factorising the walk $w=133112343442333$.}

\vspace{1mm}Initially, the walk factorisation is simply $\mathsf{Fac}\,w:=w$ and its set of \sjt{reducible factors} is therefore $S_{\!R}\big(\mathsf{Fac}\,w\big)=w$. Since $w$ is the only factor in $\mathsf{Fac}\,w$, we let $a=w$.
\sjt{Then when Algorithm \ref{AlgoCanFac} is run, the while loop beginning on line X is executed a total of Y times:}
\begin{itemize}
\item[(1)]\sjt{Since $a$ is open, we take $w_0=a$, so that $\mathsf{Fac}_0\,a=w_0$.} Traversing $w_0$ from \sjt{left to right, we find that vertex 1 is the earliest vertex visited at least twice by $w_0$. Then $s_1=13311$, $w_1=12343442333$ and $\mathsf{Fac}_1\,a=w_1\odot s_1 = 12343442333 \odot 13311$.}
\begin{itemize}
\item[(1a)]\sjt{$w_1$ is neither a simple path nor a simple cycle, and is open.} Traversing $w_1$ from its first vertex onwards \sjt{shows that vertex 2 is the} earliest vertex visited at least twice by $w_1$. Then $s_2=2343442$, $w_2=12333$ and $\mathsf{Fac}_2\,a=(w_2\odot s_2)\odot s_1$.
\item[(1b)]\sjt{$w_2$ is neither a simple path nor a simple cycle, and is open. Further, vertex 3 is the earliest vertex visited at least twice by $w_2$.} Then $s_3=333$, $w_3=123$ and $\mathsf{Fac}_3\,a=\big((w_3\odot s_3)\odot s_2\big)\odot s_1$.
\item[(1c)] \sjt{Since $w_3$ is a simple path, we exit the while loop of line XX and update $\mathsf{Fac}\,w$ by replacing $a$ by $\mathsf{Fac}_3\,a$. We thus obtain}
\begin{equation}
\mathsf{Fac}\,w=\Big((w_3\odot s_3)\odot s_2\Big)\odot s_1=\Big((123\odot333)\odot2343442\Big)\odot 13311.\nonumber
\vspace{.5mm}
\end{equation}
\end{itemize}
\item[(2)] \sjt{The set of reducible factors in $\mathsf{Fac}\,w$ is $S_{\!R}\big(\mathsf{Fac}\,w\big)=\{333,\,2343442\,,13311\}$. We return to the beginning of the while loop on Line XX, and choose $a=333$.} This walk is a cycle off 3 \sjt{and visits vertex 3 a total of $k = 3$ times. We define $c_0=33$ and $c_1=33$, and update $\mathsf{Fac}\,w$ by replacing $333$ by $33\odot 33=33^2$. The factorisation of $w$ becomes}
\begin{equation}
\mathsf{Fac}\,w=\Big((123\odot33^2)\odot2343442\Big)\odot 13311.\nonumber
\vspace{.5mm}
\end{equation}
\item[(3)] $S_{\!R}\big(\mathsf{Fac}\,w\big)=\{2343442\,,13311\}$. We choose $a=13311$. \sjt{Then $a$ is a cycle off 1 and visits vertex 1 a total of $k = 3$ times. We defin $c_0=1331$ and $c_1=11$, and update $\mathsf{Fac}\,w$ by replacing $a$ with $c_0\odot c_1$, yielding}
\begin{equation}
\mathsf{Fac}\,w=\Big((123\odot33^2)\odot2343442\Big)\odot (1331\odot11).\nonumber
\end{equation}
\item[(4)] $S_{\!R}\big(\mathsf{Fac}\,w\big)=\{2343442\,,1331\}$. \sjt{We choose $a=1331$. Now $a$ is a cycle off 1 that does not have 1 as an internal vertex. Executing the while loop on line XX results in $s_1=33$, $w_1=131$ and $\mathsf{Fac}_1\,a=w_1\odot s_1$.}
\begin{itemize}
\item[(4a)] \sjt{Since $w_1$ is a simple cycle, we exit the while loop of line XX} and update $\mathsf{Fac}\,w$, replacing $a$ with $\mathsf{Fac}_1\,a$. We obtain
\begin{equation}
\mathsf{Fac}\,w=\Big((123\odot33^2)\odot2343442\Big)\odot \Big((131\odot33)\odot 11\Big).\nonumber
\end{equation}
\vspace{.5mm}
\end{itemize}
\item[(5)] \sjt{The set of reducible factors has been reduced to $S_{\!R}\big(\mathsf{Fac}\,w\big)=\{2343442\}$. We therefore set $a=2343442$, which is a cycle off 2 that does not have 2 as an internal vertex.} Then $s_1=343$, $w_1=23442$ and $\mathsf{Fac}_1\,a=w_1\odot s_1$.
\begin{itemize}
\item[(5a)] \sjt{$w_1$ is neither a simple path nor a simple cycle, but a cycle off 2 that does not have 2 as internal vertex. Then the first pass through the while loop of line XX yields $s_2=44$, $w_2=2342$ and $\mathsf{Fac}_2\,a=(w_2\odot s_2)\odot s_1$.}
\item[(5b)] \sjt{$w_2$ is a simple cycle. We exit the while loop of line XX and update $\mathsf{Fac}\,w$, replacing $a$ with $\mathsf{Fac}_2\,a$.} We obtain
\begin{equation}\label{eq:walkFactored}
\mathsf{Fac}\,w=\bigg((123\odot 33^2)\odot \Big((2342\odot 44)\odot 343\Big)\bigg)\odot \Big((131\odot33)\odot 11\Big).
\vspace{-1mm}
\end{equation}
\end{itemize}
\end{itemize}
At this point $S_{\!R}\big(\mathsf{Fac}\,w\big)$ \sjt{is empty, and Eq.~(\ref{eq:walkFactored}) is} the prime factorisation of $w$ into nesting products of prime walks.
A pictorial representation of the operations performed by the algorithm is given \sjt{in} Fig.~\ref{fig:algo}.
\begin{figure}[t!]
\vspace{-3mm}
\hfill
\subfloat{\begin{minipage}{0.41\textwidth}
\includegraphics[width=1\textwidth]{Factor.eps}
\end{minipage}\label{fig:procedure}}
\hspace{-5mm}
\begin{minipage}{0.35\textwidth}
\subfloat{\includegraphics[width=1.2\textwidth]{TreeFactor.eps}}
\end{minipage}
\hspace{20mm}
\vspace{-4mm}
\caption{\sjt{(right) a tree $T_w$ representing} the prime factorisation of $w$. Each node corresponds to a nesting product, the leaves are the irreducible factors of $w$, and the root is the walk $w$ itself. The tree $T_w$ is in fact a subgraph of the Hasse diagram of the set of walks partially ordered by the divisibility relation of Definition \ref{def:divisibility}. This observation lies at the heart of a \sjt{``number theory" of prime walks, which will be presented in detail elsewhere.}}\label{fig:algo}
\end{figure}
\end{example}


\subsection{Prime factorisation of walk sets}\label{SectionFactorBasis}
Concluding this section on unique factorisation, we establish the factorisation of sets of walks into nested sets of primes. More precisely, we obtain \sjt{an expression for the set of all walks between any two vertices of $\G$ in terms of Kleene stars} of nested sets of simple paths and simple cycles. This result will prove decisive in the next section, when we obtain the prime representation of any series of walks.

\begin{remark}[Nesting sets]
Let $A$ and $B$ be two sets of walks on $\G$. Then we write $A\odot B$ for the set obtained by nesting every element of $B$ into every element of $A$.
\end{remark}

\begin{remark}[Kleene star and nesting Kleene star]
Let $\alpha$ be a vertex \sjt{on $\G$ and} $E_\alpha\subseteq W_{\G;\,\alpha\alpha}$ be a subset of the set of all walks from $\alpha$ to itself on $\G$. Set $E_{\alpha}^0 = \{(\alpha)\}$ and $E_{\alpha}^{i} = E_{\alpha}^{i-1}\conc E_{\alpha}$ for $i\ge 1$. Then the \emph{Kleene star} of $E_{\alpha}$, denoted $E_{\alpha}^\ast$, is the set of walks formed by concatenating any number of elements \sjt{of $E_{\alpha}$: that is,} $E_{\alpha}^{\ast}= \bigcup_{i=0}^\infty E_{\alpha}^i$ \cite{Ebbinghaus1994}. The \emph{nesting Kleene star} of $E_{\alpha}$, denoted $E_{\alpha}^{\odot\ast}$, is the equivalent of the Kleene star \sjt{with concatenation replaced} by the nesting product: $E_{\alpha}^{\odot\ast}=\bigcup_{i=0}^\infty E_{\alpha}^{\odot i}$ where $E_{\alpha}^{\odot 0}=\{(\alpha)\}$ and $E_{\alpha}^{\odot i} = E_{\alpha}^{\odot(i-1)}\odot E_{\alpha}$ for $i\geq 1$. Since nesting coincides with concatenation for cycles off the same vertex, the nesting \sjt{Kleene star coincides} with the \sjt{usual Kleene star, that is} $E_{\alpha}^{\odot\ast}=E_{\alpha}^{\ast}$. \sjt{From now on we therefore do} not distinguish between the two.
\end{remark}

\begin{theorem}[Factorisation of walk sets]\label{FactorBasis}
Let $\nu_0$ and $\nu_p$ be two vertices on $\G$. Then the set of all walks on $\G$ from $\nu_0$ to $\nu_p$ is expressible solely in terms of sets of prime walks on $\G$. This expression is \sjt{given} by the following recursive relations:
\begin{subequations}\label{eqn:FactorBasis}
\begin{align}
&W_{\G;\,\nu_0\nu_p}=\bigg(\Big(~(\,\Pi_{\G;\,\nu_0\nu_p}\odot   A^\ast_{\G\backslash\{\nu_0,\cdots,\nu_{\ell(p)-1}\};\,\nu_p})\odot\cdots\odot   A^\ast_{\G\backslash\{\nu_0\};\,\nu_1}\Big)\odot  A^\ast_{\G;\,\nu_0}\bigg)\,\label{WG},\\
\shortintertext{where $(\nu_0\,\nu_1\cdots\nu_{p-1}\,\nu_p)\in\Pi_{\G;\,\nu_0\nu_p}$ is a simple path and}
&A_{\G;\,\mu_c}=\bigg(\Big(\,(\,\Gamma_{\G;\,\mu_c}\odot   A^\ast_{\G\backslash\{\mu_c,\,\mu_1,\cdots,\,\mu_{c-2}\};\,\mu_{c-1}})\odot\cdots\odot A^\ast_{\G\backslash\{\mu_c,\,\mu_1\};\,\mu_2}\Big)\odot  A^\ast_{\G\backslash\{\mu_c\};\,\mu_1}\bigg),\label{AG}
\end{align}
\end{subequations}
with $(\mu_c\,\mu_1\cdots\mu_{c-1}\,\mu_c)\in\Gamma_{\G;\,\mu_c}$ is a simple cycle.
%If $\mathcal{V}(\G)=\varnothing$, i.e. $\G$ has not vertex, then we let $A_\G=\varnothing$.
\end{theorem}

\noindent Note that if $\nu_0=\nu_p$, \sjt{then $\Pi_{\G;\,\nu_0\nu_0}=\big\{(\nu_0)\big\}$} and $W_{\G;\,\nu_0\nu_0}=A_{\G;\,\nu_0}^\ast$ with $A_{\G;\,\nu_0}$ given by Eq.~(\ref{AG}). \sjt{This is the factorisation of sets of cycles on $\G$.}


\vspace{2mm}The set $A_{\G;\,\mu_c}$ is defined recursively through Eq.~(\ref{AG}). Indeed $A_{\G;\,\mu_c}$ is expressed in terms of $A_{\G\backslash\{\mu_c,\,\mu_1,\cdots,\,\mu_{j-1}\};\,\mu_{j}}$ which is in turn defined through Eq.~(\ref{AG}) but on the subgraph $\G\backslash{\{\mu_c,\ldots,\mu_{j-1}}\}$ of $\G$. The recursion stops when vertex $\mu_j$ has no neighbour on this subgraph, in which case $A_{\G\backslash\{\mu_c,\,\mu_1,\cdots,\,\mu_{j-1}\};\,\mu_{j}}=\Gamma_{\G\backslash\{\mu_c,\,\mu_1,\cdots,\,\mu_{j-1}\};\,\mu_{j}}=\{(\mu_j\mu_j)\}$ if the loop $(\mu_j\mu_j)$ exists and \sjt{$A_{\G\backslash\{\mu_c,\,\mu_1,\cdots,\,\mu_{j-1}\};\,\mu_{j}}=\big\{(\mu_j)\big\}$ otherwise.}
%$\matr{F}_{\mathcal{G}}[\alpha]$ is thus a matrix continued fraction which terminates at a finite depth. It is an effective weight associated to vertex $\alpha$ resulting from the dressing of $\alpha$ by all the closed walks off $\alpha$ on $\mathcal{G}$.
The maximum depth at which this recursion stops is discussed in \S \ref{StarHeightsection}.
%It characterises the structural complexity of the digraph.

%$\blacktriangleright$ Theorem \ref{FactorBasis} is proven in \S \ref{SumProof} and examples of its use are given in \S\ref{shortexmp}.
\begin{proof}
Let $\nu_0$ and $\nu_p$ be two connected vertices of $\G$, and consider $w$ a walk from $\nu_0$ to $\nu_p$.
For convenience, we define
\begin{align}
B_{\G;\,\nu_0\nu_p}&:=\bigg(\Big(~(\,\Pi_{\G;\,\nu_0\nu_p}\odot   C^\ast_{\G\backslash\{\nu_0,\cdots,\nu_{p-1}\};\,\nu_p})\,\odot\cdots\odot   C^\ast_{\G\backslash\{\nu_0\};\,\nu_1}\Big)\odot  C^\ast_{\G;\,\nu_0}\bigg),
%,\label{WG2},\\
%C_{\G;\,\mu_c}&=\bigg(\Big(~(\,\Gamma_{\G;\,\mu_c}\odot   C^\ast_{\G\backslash\{\mu_c,\,\mu_1,\cdots,\,\mu_{c-2}\};\,\mu_{c-1}})\,\odot\cdots\odot A^\ast_{\G\backslash\{\mu_c,\,\mu_1\};\,\mu_2}\Big)\odot  A^\ast_{\G\backslash\{\mu_c\};\,\mu_1}\bigg)\,\label{AG2}.
\end{align}
where $C_{\G\backslash\{\nu_0,\cdots,\nu_{j-1}\};\,\nu_j}$ designates the set of cycles off $\nu_j$ on $\G\backslash\{\nu_0,\cdots,\nu_{j-1}\}$ that do not have $\nu_j$ \sjt{as an internal vertex.}
First, we will show that $B_{\G;\,\nu_0\nu_p}=W_{\G;\,\nu_0\nu_p}$ by showing that $W_{\G;\,\nu_0\nu_p}\subseteq B_{\G;\,\nu_0\nu_p}$ and $B_{\G;\,\nu_0\nu_p}\subseteq W_{\G;\,\nu_0\nu_p}$. In a second time, we will show that $C_{\G;\,\mu_c}$ identifies with the set $A_{\G;\,\mu_c}$ defined recursively in \sjt{Theorem \ref{FactorBasis}.}

\vspace{.5mm}By Eq.~(\ref{eq:FactorW}), $w$ can be expressed as a simple path $r\in \Pi_{\G;\,\nu_0\nu_p}$ with \sjt{a collection of cycles $s_{j}$ nested into it:} that is
$\mathsf{Fac}\,w:=\big(~((r\odot s_{m})\odot s_{m-1})\odot\cdots\big)\odot s_1$ is a valid factorisation of $w$.
By construction, the $s_j$ \sjt{for $1 \le j \le m$ are cycles} nested off different vertices of the simple path $r$. \sjt{For each vertex} $\nu_k$ of $r$, we define $s_{\nu_k}=(\nu_k)$ if no $s_j$ is nested off $\nu_k$ and $s_{\nu_k}=s_j$ if $h(s_j)=\nu_k$. Then let
\begin{equation}\label{factoriDEMO}
F'(w):=\Big(~\big((r\odot s_{\nu_p})\odot s_{\nu_{p-1}}\big)\odot\cdots\Big)\odot s_{\nu_0},
\end{equation}
and note that $F'(w)\equiv \mathsf{Fac}\,w$.
By the nestable property, $s_{\nu_j}$ cannot visit \sjt{any of $\nu_0,\cdots,\nu_{j-1}$} and must therefore \sjt{be an element of $W_{\G\backslash\{\nu_0,\cdots,\nu_{j-1}\};\,\nu_j\nu_j}$.} By Eq.~(\ref{cycleSPLIT}), \sjt{any element of} $W_{\G\backslash\{\nu_0,\cdots,\nu_{j-1}\};\,\nu_j\nu_j}$ can be decomposed into nesting products of shorter cycles $c_i$ off $\nu_j$ that do not have $\nu_j$ \sjt{as an internal vertex.} Therefore  $s_{\nu_j}\in C_{\G\backslash\{\nu_0,\cdots,\nu_{j-1}\};\,\nu_j}^\ast$ and \sjt{consequently $w\in B_{\G;\,\nu_0\nu_p}$. Since $w$ was arbitrary, it follows that $W_{\G;\,\nu_0\nu_p}\subseteq B_{\G;\,\nu_0\nu_p}$.} Furthermore, any element of $B_{\G;\,\nu_0\nu_p}$ is a walk on $\G$ from $\nu_0$ to $\nu_p$\sjt{, so that $B_{\G;\,\nu_0\nu_p}\subseteq W_{\G;\,\nu_0\nu_p}$.} Hence we deduce $B_{\G;\,\nu_0\nu_p}= W_{\G;\,\nu_0\nu_p}$.

\vspace{.5mm}It remains to show that $C_{\G;\,\mu_c}$ is the set $A_{\G;\,\mu_c}$ of \sjt{Eq.~\eqref{eqn:FactorBasis}}. Let $c\in C_{\G;\,\mu_c}$. Applying the same reasoning as above, $c$ factorises as in Eq.~(\ref{factoriDEMO}), but with \sjt{$r$ being a simple cycle (i.e.~an element of $\Gamma_{\G;\,\mu_c}$) instead of a simple path. Thus $c$ is an element of the set}
\begin{equation}\label{ensemright}
\bigg(\Big(~(\,\Gamma_{\G;\,\mu_c}\odot   C^\ast_{\G\backslash\{\mu_c,\,\mu_1,\cdots,\,\mu_{c-2}\};\,\mu_{c-1}})\,\odot\cdots\odot C^\ast_{\G\backslash\{\mu_c,\,\mu_1\};\,\mu_2}\Big)\odot  C^\ast_{\G\backslash\{\mu_c\};\,\mu_1}\bigg).
\end{equation}
\sjt{Any element of this set is a cycle off $\mu_c$ that does not have $\mu_c$ as an internal vertex. Consequently, $C_{\G;\,\mu_c}$ identifies with the set of Eq.~(\ref{ensemright}). If $\mu_c$ has no neighbour on $\G$, then $C_{\G;\,\mu_c}=\big\{(\mu_c\mu_c)\big\}$ if the loop $(\mu_c\mu_c)$ exists and $C_{\G;\,\mu_c}=\big\{(\mu_c)\big\}$} otherwise. \sjt{Thus since $C_{\G;\,\mu_c}$ and $A_{\G;\,\mu_c}$ both fulfill the same recursive relation and value on vertices with no neighbour, it follows that they are equal.}  This establishes Eq.~(\ref{AG}) and, together with $B_{\G;\,\nu_0\nu_p}= W_{\G;\,\nu_0\nu_p}$, Eq.~(\ref{WG}). \qed
\end{proof}

\vspace{2mm}\begin{example}[Prime factorisation of a walk set]\label{exampleK3}
\sjt{Let $\mc{T}_{3}$ be the complete graph on three vertices, with a self-loop on each vertex. We label the vertices 1, 2, and 3. In this example we derive the prime factorisation of the set of all walks from 1 to 1 on $\mc{T}_3$.}
\sjt{The set of all walks from 1 to 1 is a set of cycles, and Eq.~(\ref{WG}) thus yields} $W_{\mc{T}_{3};\,11}=A_{\mc{T}_{3};\,11}^\ast$. To factorise $A_{\mc{T}_{3};\,11}^\ast$, we note that the set of simple cycles from 1 to itself \sjt{is $\Gamma_{\mc{T}_{3};\,1}=\{11,121,131,1231,1321\}$.} Thus Eq.~(\ref{AG}) gives
\begin{align}\label{FactorW11K3step1}
W_{\mc{T}_{3};\,11}&=\bigg\{11,\,121\odot A^\ast_{\mc{T}_{3}\backslash\{1\};\,22},\,131\odot A^\ast_{\mc{T}_{3}\backslash\{1\};\,33},\\
&\hspace{0mm}\big(1231\odot A^\ast_{\mc{T}_{3}\backslash\{1,2\};\,33}\big)\odot A^\ast_{\mc{T}_{3}\backslash\{1\};\,22},\,\big(1321\odot A^\ast_{\mc{T}_{3}\backslash\{1,3\};\,22}\big)\odot A^\ast_{\mc{T}_{3}\backslash\{1\};\,33}\bigg\}^\ast.\nonumber
\end{align}
We now \sjt{use Eq.~(\ref{AG}) to factor each of the sets $A^\ast_{\G;\mu\mu}$.} Since \sjt{$\Gamma_{\mc{T}_{3}\backslash\{1\};\,2}=\{22,232\}$ and $\Gamma_{\mc{T}_{3}\backslash\{1,3\};\,2}=\{22\}$,} we have
\begin{equation}\label{FactorW11K3step2}
A^\ast_{\mc{T}_{3}\backslash\{1\};\,22}=\{22,232\odot A^\ast_{\mc{T}_{3}\backslash\{1,2\};\,33}\}^\ast\quad\text{and}\quad A^\ast_{\mc{T}_{3}\backslash\{1,3\};\,22}=\{22\}^\ast,
\end{equation}
and the analogous expressions produced by exchanging the labels $2$ and $3$. Inserting these
expressions into Eq.~(\ref{FactorW11K3step1}), we arrive at
\begin{align}\label{W11K3Factor}
W_{\mc{T}_{3};\,11}=\bigg\{&11,121\odot\Big\{22,232\odot\{33\}^\ast\Big\}^\ast,\,131\odot\Big\{33,323\odot\{22\}^\ast\Big\}^\ast,\\
&\hspace{-5mm}\big(1231\odot\{33\}^\ast\big)\odot\Big\{22,232\odot\{33\}^\ast\Big\}^\ast,\,\big(1321\odot\{22\}^\ast\big)\odot\Big\{33,323\odot\{22\}^\ast\Big\}^\ast\bigg\}^\ast.\nonumber
\end{align}
This set contains the prime factorisation of any cycle off $1$ on $\mc{T}_3$.
%The star height of the prime factorisation of $W_{\mc{T}_{3};\,11}$ is 3, as predicted by Theorem \ref{StarHeighGraph}.
\end{example}

\section{Prime factorisation of series of walks}\label{PathSumPrimeSeries}
The main interest of the existence and uniqueness of the prime factorisation of walks \sjt{is that it permits a series of walks on a digraph $\G$ to be resummed into an expression that involves only the prime elements of $\G$.} This is analogous to how the fundamental theorem of arithmetic \sjt{leads to the existence} of Euler products for the Riemann zeta function and other totally multiplicative \sjt{functions on the integers}. In fact, \sjt{as we will show in a future work,} the relation between these two cases is not simply an analogy but can be established rigorously.

In this section, we begin by obtaining an explicit closed-form expression involving only prime walks for the formal series of all walks on the graph. \sjt{We also obtain the equivalent expression for series of walk weights on a weighted directed graph. These resummed walk series have found applications} in linear algebra \cite{Giscard2011b}, machine learning \cite{Malioutov2006} and physics \cite{Brydges1983}.

\subsection{Formal series of walks}\label{formal}
Let $\alpha$ and $\omega$ be two vertices on $\G$. The \emph{characteristic series} of the set $W_{\G;\,\alpha\omega}$ of all walks from $\alpha$ to $\omega$ on $\G$ is the formal series \cite{Berstel2008}
\begin{equation}
\Sigma_{\G;\,\alpha\omega}:=\sum_{w\in W_{\G;\,\alpha\omega}} w.
\end{equation}
In other words, the coefficient of $w$ in $\Sigma_{\G;\,\alpha\omega}$, denoted $(\Sigma_{\G;\,\alpha\omega},w)$, is 1 if $w\in W_{\G;\,\alpha\omega}$ and 0 otherwise.
%If it exists, the weighted characteristic series $\W[\Sigma_{\G;\,\alpha\omega}]$ is the series of all walk weights.

%The results of this section are proven in \S \ref{SumProof}

%We now use Theorem \ref{FactorBasis} to factor the sum of all the walks $w$ between any two vertices $(\alpha,\omega)\in\mathcal{V}(\G)$, denoted by $\Sigma_{\mathcal{G};\alpha\omega}$.
By using the fact that every open walk can be factorised into a simple path and a collection of nested cycles, we rewrite $\Sigma_{\G;\,\alpha\omega}$ as a series over simple paths by modifying each path in the series to include all collections of cycles that can be nested off the vertices it visits. To preserve the vertex-edge notation of walks, we implement this modification by replacing each vertex $\alpha$ in a simple path by a `dressed vertex' $(\alpha)'_{\G}$ defined to represent the characteristic series of all cycles that can be nested off $\alpha$ on $\G$:
\begin{equation}\label{DressedVertex}
(\alpha)'_{\G}:=\sum_{c\,\in\, W_{\G;\,\alpha\alpha}}c=\Sigma_{\G;\,\alpha\alpha}.
\end{equation}
\sjt{We rewrite this characteristic series as a series over simple cycles $\gamma\in\Gamma_{\G;\,\alpha}$ by replacing each vertex $\mu$ visited} by a simple cycle $\gamma$ by a dressed vertex representing the characteristic series of all the cycles that can be nested off $\mu$ on the appropriate subgraph of $\G$. \sjt{Applying this approach recursively yields} a representation of the formal series $\Sigma_{\G;\,\alpha\omega}$ which only involves simple paths and simple cycles \sjt{(i.e.~the prime walks on $\G$).}

%Using the vertex-edge notation of walks, the dressed vertex is therefore
%\begin{align}\label{DressedVertex2}
%(\alpha)'_{\G}&=\sum_{p\in\mathbb{N}}\left(\sum_{(\alpha\mu_2\cdots\mu_m\alpha)\,\in\, \Gamma_{\G;\,\alpha}}(\alpha)(\alpha\mu_2)(\mu_2)'_{\G\backslash\{\alpha\}}\cdots (\mu_m)'_{\G\backslash\{\alpha,\,\mu_2,\cdots,\mu_{m-1}\}}(\mu_m\alpha)(\alpha)\right)^p,\nonumber\\
%&=\sum_{p\in\mathbb{N}}\Big(\sum_{\gamma\in\Gamma_{\G;\,\alpha}}\gamma'\Big)^p,
%\end{align}
%where the sums over $p\in\mathbb{N}$ account for cycles made of a single repeated simple cycle, e.g. $\gamma^p$, and $\gamma'$ is a notation for a simple cycle $\gamma$ with dressed vertices.
%%
%This procedure is an implementation of the recursive formulation of Eqs.~(\ref{WG}, \ref{AG}).
%Finally, we show in \S \ref{SumProof} that the linear mapping representing a dressed vertex on the quiver is the inverse mapping $\varphi_{(\alpha)'_{\G}}=\big(1_{\alpha}-\sum_{\gamma\in\Gamma_{\G;\,\alpha}}\varphi_{\gamma'}\big)^{-1}$ and from now on we represent dressed vertices using the inverse notation.

\begin{theorem}[Formal path-sum]\label{FactorSum}
Using the vertex-edge notation for walks, the formal characteristic series of all walks from $\alpha$ to $\omega$ on $\G$ has the following \sjt{expression, which involves only primes on $\G$:}
\begin{subequations}
\begin{align}\label{eqn:SumOfAllWalks}
\Sigma_{\G;\,\alpha\omega}=\sum_{\Pi_{\G;\,\alpha\omega}}\left(\alpha\right)'_\G\left(\alpha\nu_2\right) \left(\nu_2\right)'_{\G\backslash\{\alpha\}} \cdots (\nu_{\ell(p)}\omega)\left(\omega\right)'_{\G\backslash\{\alpha,\nu_2,\ldots,\nu_{\ell(p)}\}},
\end{align}
where $p=(\alpha\nu_2\cdots\nu_{\ell(p)}\omega)$ is a simple path of length $\ell(p)$ from $\alpha$ to $\omega$, and $\left(\alpha\right)'_\G$ denotes the dressed vertex $\alpha$ on $\G$, defined as the formal series of all cycles off $\alpha$ on $\G$ and given explicitly by
\begin{equation}
\left(\alpha\right)'_\G
=\Bigg[\left(\alpha\right) -\sum_{\gamma\in\Gamma_{\G;\,\alpha}}
 \left(\alpha\right)\left(\alpha\mu_2\right)\left(\mu_2\right)'_{\G\backslash\{\alpha\}}\left(\mu_2\mu_3\right)\cdots(\mu_{\ell(\gamma)})'_{\G\backslash\{\alpha,\mu_2,\ldots,\mu_{\ell(\gamma)-1}\}} (\mu_{\ell(\gamma)}\alpha)(\alpha)\Bigg]^{-1},\label{eqn:DressedVertexClosedForm2B}
\end{equation}
\end{subequations}
with $\gamma=(\alpha\mu_2\cdots\mu_{\ell(\gamma)}\alpha)$ a simple cycle of length $\ell(\gamma)$ off $\alpha$.
%\begin{subequations}
%\begin{align}
%&\Sigma_{\G;\,\alpha\omega}=\sum_{p\in \Pi_{\G;\,\alpha\omega}}\Sigma_{\G;\,\alpha\alpha}\prod_{j=1}^{\ell(p)}\bigg\{(\nu_{j}\nu_{j+1})\,\Sigma_{\G\backslash\{\alpha,\nu_2,\cdots,\nu_{j-1}\};\,\nu_{j}\nu_{j}}\bigg\},\\
%&\Sigma_{\G;\,\alpha\alpha}=\left[1-\sum_{\gamma\in\Gamma_{\G;\,\alpha\alpha}}\prod_{j=1}^{\ell(\gamma)}\bigg\{
%\Sigma_{\G\backslash\{\alpha,\,\mu_1,\,\cdots,\,\mu_{j-1}\};\,\mu_{j}\mu_{j}}\, (\mu_j\mu_{j-1})\bigg\}\right]^{-1},\label{seriescompact}
%\end{align}
%\end{subequations}
%where the products are left-to-right,
%Equivalently, on expanding the products $\Sigma_{\G;\,\alpha\omega}$ has the explicit form
%\begin{subequations}
%\begin{align}\label{eqn:SumOfAllWalks}
%&\Sigma_{\G;\,\alpha\omega}=\sum_{p\in\Pi_{\G;\,\alpha\omega}}\Sigma_{\G;\,\alpha\alpha}\left(\alpha\nu_2\right) \Sigma_{\G\backslash\{\alpha\};\,\nu_2\nu_2} \cdots (\nu_{\ell(p)}\omega)\,\Sigma_{\G\backslash\{\alpha,\nu_2,\ldots,\nu_{\ell(p)}\};\,\omega\omega},\\
%\end{align}
%where $p$ is the length of the simple path $(\alpha\nu_2\cdots\nu_p\omega) \in \Pi_{\G;\,\alpha\omega}$, and $\left(\alpha\right)'_\G$ denotes the dressed vertex $\alpha$ on $\G$, given by
%\begin{equation}
%&\Sigma_{\G;\,\alpha\alpha}
%=\Bigg[\left(\alpha\right) -\sum_{\Gamma_{\G;\,\alpha}}
% \left(\alpha\right)\left(\alpha\mu_2\right)\left(\mu_2\right)'_{\G\backslash\{\alpha\}}\left(\mu_2\mu_3\right)\cdots\left(\mu_{\ell(\gamma)}\right)'_{\G\backslash\{\alpha,\mu_2,\ldots,\mu_{{\ell(\gamma)}-1}\}} \left(\mu_{\ell(\gamma)}\alpha\right)\Bigg]^{-1},\label{eqn:DressedVertexClosedForm2B}
% \end{align}
%\end{subequations}
\end{theorem}
\sjt{The formal series $\Sigma_{\G;\alpha\omega}$ is expressed recursively in terms of formal series on subgraphs of $\G$. We term these formal series the dressed vertices, and denote them by e.g.~ $(\mu_{j})'_{\G\backslash\{\alpha,\,\mu_1,\,\cdots,\,\mu_{j-1}\}}$. These subseries are in turn obtained through Eq.~(\ref{eqn:DressedVertexClosedForm2B}), but on the subgraphs of $\G$ (e.g. $\G\backslash\{\alpha,\mu_2,\ldots,\mu_{j-1}\}$ in the case of $(\mu_{j})'_{\G\backslash\{\alpha,\,\mu_1,\,\cdots,\,\mu_{j-1}\}}$.)} The recursion stops when vertex $\mu_j$ has no neighbour on this subgraph. \sjt{In this case the dressed vertex is given by
\begin{align}
  (\mu_{j})'_{\G\backslash\{\alpha,\,\mu_1,\,\cdots,\,\mu_{j-1}\}}=\sum_{n\geq0}(\mu_j\mu_j)^n= \begin{cases}
    [(\mu_j)-(\mu_j\mu_j)]^{-1}&\text{if the loop $(\mu_j\mu_j)$ exists},\\
    (\mu_j) & \text{otherwise,}
  \end{cases}
\end{align}
where $(\mu_j)$ is the trivial walk off the vertex $\mu_j$.}\\

\vspace{1mm}The recursive nature of Eq.~(\ref{eqn:DressedVertexClosedForm2B}) implies that the result of Theorem \ref{FactorSum} for $\Sigma_{\G;\,\alpha\omega}$ yields a formal continued fraction involving only prime walks. On finite digraphs, the depth of this continued fraction is finite but determining its precise value is difficult, \sjt{as we discuss further in \S\ref{StarHeightsection}.}

\begin{proof}
\sjt{Theorem \ref{FactorSum}} follows from the factorisation of sets of walks into nested sets of primes presented in Theorem \ref{FactorBasis}. We provide two proofs of the theorem, one based on  formal series, the other on quivers.

\textit{Proof 1} \sjt{Consider the set of all walks from $\alpha$ to $\omega$ on $\G$, denoted by $W_{\G;\,\alpha\omega}$.} We first decompose $W_{\G;\,\alpha\omega}$ using Eq.~(\ref{WG}), identifying $\alpha$ with $\nu_0$ and $\omega$ with $\nu_{\ell(p)}$ for convenience, then sum over the elements of the sets on both sides of the equality. This yields, in vertex-edge notation,
\begin{align}\label{SumStep0}
\Sigma_{\G;\,\alpha\omega}&=\sum_{p\in \Pi_{\G;\,\alpha\omega}}\left(\sum_{\mathfrak{a}_1\in A^\ast_{\G;\,\alpha}}\mathfrak{a}_1\right)(\alpha\nu_2)\left(\sum_{\mathfrak{a}_2\in A^\ast_{\G\backslash\{\alpha\};\,\nu_2}}\mathfrak{a}_2\right)(\nu_2\nu_3)\cdots\\
&\hspace{55mm}\cdots(\nu_{\ell(p)}\omega)\left(\sum_{\mathfrak{a}_{\ell(p)+1}\in A^\ast_{\G\backslash\{\alpha,\nu_1,\cdots,\nu_{\ell(p)}\};\,\omega}}\mathfrak{a}_{\ell(p)+1}\right),\nonumber
\end{align}
which we obtain upon nesting the sets $A^\ast_{\G;\,\alpha},\,A^\ast_{\G\backslash\{\alpha\};\,\nu_2},\ldots$ into the \sjt{simple path $p = \alpha\nu_2\cdots\nu_{\ell(p)}\omega \in \Pi_{\G;\,\alpha\omega}$} at the appropriate positions. Equation (\ref{SumStep0}) shows that \sjt{the sum over each of these sets gives rise to an `effective vertex', which is produced by dressing a `bare vertex' $\nu_j$ by all cycles that visit it on the subgraph $\G\backslash\{\alpha,\ldots,\nu_{j-1}\}$. Motivated by this observation, we therefore define the vertex $\alpha$ dressed by cycles on $\G$, denoted by $(\alpha)'_{\G}$, to be the formal series}
\begin{equation}\label{Dress}
(\alpha)'_{\G}:=\sum_{\mathfrak{a}_1\in A^\ast_{\G;\,\alpha}}\mathfrak{a}_1.
\end{equation}
It follows that Eq.~(\ref{SumStep0}) yields Eq.~\eqref{eqn:SumOfAllWalks}, with dressed vertices representing the characteristic series \sjt{of the sets $A^\ast_{\G\backslash\{\alpha,\nu_1\cdots \nu_{j-1}\};\,\nu_j}$.} These series are proper \cite{Droste2009}: their constant term is a \sjt{trivial walk (e.g. $(\alpha)$ in Eq.~(\ref{Dress}))} which is different from 0. Thus the series represent formal inverses \cite{Sakarovitch2009}, e.g. $(\alpha)'_{\G}=[(\alpha)-\sum_{\mathfrak{a}_1\in A_{\G;\,\alpha}} \mathfrak{a}_1]^{-1}$. Note that the sum appearing in the inverse runs over $A_{\G;\,\alpha}$ rather than its Kleene star, showing that the inverse is \sjt{a representation of the characteristic series of $A^\ast_{\G;\,\alpha}$ as an geometric series in the characteristic series of $A_{\G;\,\alpha}$}.

By combining these results with Eq.~(\ref{AG}), the dressed vertices are seen to be of the form
  \begin{align}
  \left(\alpha\right)'_\G  & =\Bigg[(\alpha)-\sum_{\Gamma_{\G;\alpha}}(\alpha)\left(\alpha\mu_2\right)(\mu_2)'_{\G\backslash\{\alpha\}}\left(\mu_2\mu_3\right)\cdots \left(\mu_m\alpha\right)\Bigg]^{-1},\label{SumOverKleeneStars}
\end{align}
\sjt{where $\alpha\mu_2\cdots\mu_{\ell(\gamma)}\omega$ is a simple cycle} and $(\alpha)$ is the local identity common to all walks of $W_{\G;\alpha\alpha}$: for any cycle $c$ off $\alpha$, we have $c^0=(\alpha)$. In this expression, the dressed vertices again represent sums over the Kleene stars that appear when $A_{\G;\,\alpha}$ is decomposed using Eq.~(\ref{AG}). This establishes Eq.~(\ref{eqn:DressedVertexClosedForm2B}).\qed

\textit{Proof 2} We obtain the same results explicitly with the help of quivers. Let $\mathfrak{V}=\{V\}$ be a collection of vector spaces, each of arbitrary finite dimension, such that $\mathfrak{V}$ is in one to one correspondence with the vertex set $\mc{V}(\G)$ of the finite directed graph $\G$. For simplicity we designate by $V_\mu\in\mathfrak{V}$ the vector space associated to vertex $\mu\in\mc{V}(\G)$. Let $\mathfrak{F}=\{\varphi_{\nu\ot\mu}:V_\mu\to V_\nu\}$ be a collection of linear mappings in one to one correspondence with the edge set $\mc{E}(\G)$ of $\G$. We associate the linear mapping $\varphi_{\nu\ot\mu}\in\mathfrak{F}$ to the directed edge from $\mu$ to $\nu$.
Then $\mathfrak{G}=(\mathfrak{V},\,\mathfrak{F})$ is a representation of the directed graph $\G$, which in this context is also called a \emph{quiver} \cite{Dersken2005,Savage2005}. The representation of a walk \sjt{$w=(\alpha_1\alpha_2\cdots\alpha_{\ell(w)}+1)\in W_\G$ }is the linear mapping $\varphi_w$ obtained from the composition of the linear mappings representing the successive edges traversed by the \sjt{walk: that is,} $\varphi_w=\varphi_{\alpha_{\ell}\ot\alpha_{\ell-1}}\conc\cdots\conc\varphi_{\alpha_3\ot\alpha_2}\conc\varphi_{\alpha_{2}\ot\alpha_1}$. The representation of a \sjt{trivial walk $(\mu)$ is the identity map $1_{\mu}$ on $V_\mu$, and the representation of the empty walk $0$ is the 0 map.}

Now \sjt{define $\varphi_{\Gamma_{\G;\,\alpha}}$ to be the} mapping representing the finite series $\sum_{\gamma\in\Gamma_{\G;\,\alpha}}\gamma'$. By linearity, \sjt{we have} $\varphi_{\Gamma_{\G;\,\alpha}}=\sum_{\gamma\in\Gamma_{\G;\,\alpha}}\varphi_{\gamma'}$.
Define $\varphi_{(\alpha)'_{\G}}=\sum_{p\in\mathbb{N}}\varphi_{\Gamma_{\G;\,\alpha}}^{(p)}$, where $\varphi_{\Gamma_{\G;\,\alpha}}^{(p)}$ is the $p$-th composition of $\varphi_{\Gamma_{\G;\,\alpha}}$ with itself, $\varphi_{\Gamma_{\G;\,\alpha}}^{(0)}$ being the local identity map $1_{\alpha}$. Then observe that
$\varphi_{(\alpha)'_{\G}}\conc\varphi_{\Gamma_{\G;\,\alpha}}=\varphi_{\Gamma_{\G;\,\alpha}}\conc\varphi_{(\alpha)'_{\G}}=\sum_{p\in\mathbb{N}}\varphi_{\Gamma_{\G;\,\alpha}}^{(p+1)}=\varphi_{(\alpha)'_{\G}}-1_{\alpha}$. Consequently, $\varphi_{(\alpha)'_{\G}}$ is the compositional inverse
\begin{equation}
\varphi_{(\alpha)'_{\G}}=\big(1_{\alpha}-\varphi_{\Gamma_{\G;\,\alpha}}\big)^{(-1)},
\end{equation}
which is the quiver representation of the formal inverse representation of a dressed vertex $(\alpha)'_{\G}=[(\alpha)-\sum_{c\in A_{\G;\,\alpha}} c]^{-1}$.\qed
% By the same token, the matrix representation of $\varphi_{(\alpha)'_{\G}}$ is the matrix inverse of the matrix representation of $1_{\alpha}-\varphi_{\Gamma_{\G;\,\alpha}}$.
\end{proof}


\vspace{2mm}\begin{example}[Formal series of walks on a digraph]\label{FactorExample} Let $\G$ be the digraph illustrated \sjt{in Fig. \ref{fig:GRef},} and consider the formal series $\Sigma_{\G;\,11}$ of all walks from vertex 1 to itself on $\G$.
\begin{figure}[t!]
\begin{center}
\vspace{-2mm}
\includegraphics[width=.5\textwidth]{GraphReferee.eps}
\vspace{-3mm}
\caption[Digraph of Example \ref{FactorExample}]{The digraph $\mc{G}$ of Example \ref{FactorExample}.}
\label{fig:GRef}
\end{center}
\vspace{-2mm}
\end{figure}
Theorem \ref{FactorSum} yields this series as
\begin{equation}
\Sigma_{\G;\,11}=\Big[(1)-(11)-(12)(2)'_{\G\backslash\{1\}}(231)\Big]^{-1},
\end{equation}
where we used that the set of simple cycles off 1 on $\G$ is $\Gamma_{\G;\,11}=\{(11),(1231)\}$ and $\Gamma_{\G\backslash\{1,2\};33}$ is \sjt{empty, so that $(3)'_{\G\backslash\{1,2\}}=(3)$ is trivial.} We obtain the dressed vertex $(2)'_{\G\backslash\{1\}}$, which represents the sum of all cycles off $2$ on $\G\backslash\{1\}$, thanks to Eq.~(\ref{eqn:DressedVertexClosedForm2B}) as
\begin{subequations}
\begin{align}
(2)'_{\G\backslash\{1\}}&=\Big[(2)-(24)(4)'_{\G\backslash\{1,2\}}(42)\Big]^{-1},\\
\shortintertext{since $\Gamma_{\G\backslash\{1\};22}=\{(242)\}$. Similarly,}
(4)'_{\G\backslash\{1,2\}}&=\Big[(4)-(44)-(4564)\Big]^{-1},
\end{align}
\end{subequations}
on using that $\Gamma_{\G\backslash\{1,2\};44}=\{(44),(4564)\}$ and the sets $\Gamma_{\G\backslash\{1,2,4\};55}$ and $\Gamma_{\G\backslash\{1,2,4,5\};66}$ are empty. Finally,
\begin{equation}
\Sigma_{\G;\,11}=\left[(1)-(11)-(12)\left[(2)-(24)\Big[(4)-(44)-(4564)\Big]^{-1}(42)\right]^{-1}(231)\right]^{-1}.
\end{equation}
This expression for $\Sigma_{\G;\,11}$ is recovered upon summing over the prime factorised form for the set of all walks from 1 to itself \sjt{on $\G$, namely}
\begin{equation}\label{WG11exFact}
W_{\G;\,11}=\Big\{11,\,1231\odot\big\{242\odot\{44,\,4564\}^\ast\big\}^\ast\Big\}^\ast.
\end{equation}
\end{example}

\subsection{Prime factorisations of weighted sums of walks}\label{weightedsum}
We now consider the weighted counterparts \sjt{of formal walk series,} which arise when summing walks on weighted digraphs. Evidently, \sjt{series of walk weights, rather than formal series of walks, are the objects found in applications.}

A \emph{weighted digraph} $(\G,\W)$ is a digraph $\G$ paired with a weight function $\W$ that assigns a weight $\W[e]$ to each directed edge $e$ of $\G$. For the sake of generality we let the weight of a directed edge from $\mu$ to $\nu$, denoted $\ew_{\nu\mu} := \W[(\mu\nu)]$, be a $d_\nu$-by-$d_\mu$ complex matrix.% representing the linear mapping $\varphi_{\nu\ot\mu}$.
\sjt{We extend the action of $\W$ from edges to walks by defining the weight of a trivial walk $(\mu)$ to be the $d_\mu \times d_\mu$ identity matrix $\I_\mu$, and the weight of a walk $w = \alpha\mu_2\cdots\mu_L\omega$ of length $L \ge 1$ to be the right-to-left product of the weights of the edges traversed by $w$: $\W[w] = \W[(\mu_L\omega)]\cdots\W[(\alpha\mu_2)]$. Note that the ordering of the edge weights is suitable for the matrix multiplications to be carried out, the end result being a $d_\omega \times d_\alpha$ matrix. }

\begin{corollary}[Path-sum expression of weighted sums of walks]\label{FactorSumOfWeights}
\sjt{Let $(\G,\W)$ be a weighted digraph, and $\alpha$ and $\omega$ be two vertices on $\G$.
If it exists, sum of the weights of all walks from $\alpha$ to $\omega$ on $\G$, denoted by $\W\,\Big[\Sigma_{\G;\,\alpha\omega}\Big]=\sum_{w\in W_{\G;\alpha\omega}} \W[w]$, admits a factorised form involving only the weights of prime walks. We term this form a path-sum representation. It is explicitly given by}
\begin{subequations}
\begin{align}
&\W\,\Big[\Sigma_{\G;\,\alpha\omega}\Big]=\sum_{p\in \Pi_{\G;\,\alpha\omega}}\prod_{j=1}^{\ell(p)+1}\bigg\{\W\,\Big[\Sigma_{\G\backslash\{\alpha,\,\nu_2,\cdots,\,\nu_{j-1}\};\,\nu_{j}\nu_{j}}\Big]\, \ew_{\nu_{j+1}\nu_{j}}\bigg\}\,\W\,\Big[\Sigma_{\G;\,\alpha\alpha}\Big]\,,\\
&\W\,\Big[\Sigma_{\G;\,\alpha\alpha}\Big]=\left(1-\sum_{\gamma\in\Gamma_{\G;\,\alpha\alpha}}\ew_{\mu_{1}\mu_{\ell(\gamma)}}\prod_{j=2}^{\ell(\gamma)}\bigg\{
\W\,\Big[\Sigma_{\G\backslash\{\alpha,\,\mu_2,\cdots,\,\mu_{j-1}\};\,\mu_{j}\mu_{j}}\Big]\, \ew_{\mu_j\mu_{j-1}}\bigg\}\right)^{-1},\label{Saa}
\end{align}
\sjt{where the products are to be constructed right-to-left; $p=\nu_1\nu_2\cdots \nu_{\ell(p)+1}$ is a simple path, where we identify $\alpha$ with  $\nu_1$ and $\omega$ with $\nu_{\ell(p)+1}$; and $\gamma=(\mu_1\mu_2\cdots \mu_{\ell_\gamma}\mu_1)$ is a simple cycle off $\alpha\equiv \mu_1$.}\\
\end{subequations}
\end{corollary}
%\vspace{-3mm}\noindent The corollary provides a recursive formula for $\W[\Sigma_{\G;\alpha\alpha}]$ since this quantity is expressed in terms of weighted sums of walks, such as $\W\big[\Sigma_{\G\backslash\{\alpha\};\mu_1\mu_1}\big]$, which in turn satisfy Eq.~(\ref{Saa}) on subgraphs of $\G$. This gives rise to a continued fraction representation of the walk sum.
\begin{proof}
The corollary is an immediate consequence of the formal results of Theorem \ref{FactorSum} on noting that the weight function is \sjt{i) linear, so that $\W\big[w+w'\big] = \W\big[w\big]+\W\big[w'\big]$, and ii) a homomorphism, so that $\W[e_1\conc e_2]=\W[e_2]\W[e_1]$ for any two directed edges $e_1$, $e_2$ such that $e_1\conc e_2$ is non-zero.}

\sjt{The corollary can alternatively be obtained by using} the quiver introduced in the proof of Theorem \ref{FactorSum}. Consider the matrix representation of the mapping $\varphi_{(\alpha)'_{\G}}$. Since $\varphi_{(\alpha)'_{\G}}$ is the inverse mapping of $1_{\alpha}-\varphi_{\Gamma_{\G;\,\alpha}}$, its matrix representation is the matrix inverse of the matrix representation of $1_{\alpha}-\varphi_{\Gamma_{\G;\,\alpha}}$.\qed
\end{proof}
\begin{remark}[Existence of the weighted path-sum]
If $\G$ has finitely many edges and vertices, it sustains only a finite number of primes and the path-sum representation of the weighted series of walks involves only finitely many terms. An immediate consequence is \sjt{that \emph{the path-sum representation exists even when the sum of walk weights diverges.} In this situation the path-sum has been shown to be the unique analytic continuation of the sum of walk weights, and remains a valid representation of this sum \cite{Giscard2011b}. This result leads to applications in the field of matrix computations.}
\end{remark}

%It follows that for $(w,w')\in W_\G^2$ such that $w\conc w'\neq0$, we have
%\begin{subequations}\label{eqn:Weightproperties}
%\begin{align}
%  \W\big[w\conc w'\big] &= \W\big[w'\big]\W\big[w\big].
%\shortintertext{Furthermore, for walks $w,\, w'$ satisfying $h(w) = h(w')$ and $t(w) = t(w')$ we define}
%  \W\big[w+w'\big] &= \W\big[w\big]+\W\big[w'\big].
%\end{align}
%\end{subequations}




%
%\begin{remark}[More general weights]\label{MatFunc}
%It is possible to generalise the definitions of quiver and of weighted digraph to the case where the weight of an edge from $\mu$ to $\nu$ is any morphism $\phi_{\nu\leftarrow\mu}:V_\mu\to V_\nu$ in an additive category $\mathcal{C}$ from an object $V_\mu$, associated with the vertex $\mu$, to an object $V_\nu$, associated with the vertex $\nu$. Then all the results of this article hold upon requiring that the matrix of morphisms $(\mathsf{M})_{\nu\mu}=\phi_{\nu\leftarrow\mu}$ be invertible. This remark is based on an observation of \cite{Gelfand2005}.
%\end{remark}




%\begin{corollary}[Weighted path-sum]\label{FactorSumOfWeights}\label{PSresult} Let $\mathsf{M}$ be an invertible matrix defined through $(\mathsf{M})_{\nu\mu}=\ew_{\nu\mu}$. Then as long as all of the required inverses exist, the weight of the sum of all walks from $\alpha$ to $\omega$ on the weighted digraph $(\G,\W)$ is given by
%\begin{subequations}\label{WeightedSum}
%\begin{align}
%\W\big[\Sigma_{\G;\,\alpha\omega}\big]&=\sum_{\Pi_{\G;\,\alpha\omega}} \matr{F}_{\G\backslash\{\alpha,\ldots,\nu_p\};\,\omega}\, \ew_{\omega\nu_p}\cdots \matr{F}_{\G\backslash\{\alpha\};\,\nu_2}\,\ew_{\nu_2\alpha}\,\matr{F}_{\G;\alpha}\,,\label{WeightedSumpath}
%\shortintertext{where $p$ is the length of the simple path, $\ew_{\nu\mu} =\W[(\mu\nu)]$ is the weight of the edge $(\mu\nu)$, and}
%\matr{F}_{\G;\,\alpha} \equiv \W\big[(\alpha)'_\G\big]
%&=\bigg[\I_\mu-\sum_{\Gamma_{\G;\,\alpha}}\,\ew_{\alpha\mu_m}\,\mathsf{F}_{\G\backslash\{\alpha,\ldots,\mu_{m-1}\};\,\mu_m}\,\ew_{\mu_m\mu_{m-1}}\cdots \mathsf{F}_{\G\backslash\{\alpha\};\,\mu_2}\,\ew_{\mu_2\alpha}\bigg]^{-1},\label{Fweights}
%\end{align}
%\end{subequations}
%with $m$ the length of the simple cycle and $\matr{I}_\mu$ the $d_\mu\times d_\mu$ identity matrix. $\matr{F}_{\G;\,\alpha}$ is the effective weight of the vertex $\alpha$ on $\G$ once it is dressed by all the cycles off it.
%\end{corollary}
%
%The expression of $\W\big[\Sigma_{\G;\,\alpha\omega}\big]$ is a continued fraction of finite depth, which results from the recursive definition of the $\mathsf{F}_{\G;\,\alpha}$. Theorem \ref{FactorSumOfWeights} thus expresses the sum of the weights of all walks from $\alpha$ to $\omega$ on any finite digraph as a \emph{finite matrix-valued continued fraction} over the simple paths and simple cycles of $\G$. As we will see with the examples, this allows direct verifications using matrix computations of the results of Theorem \ref{FactorSum} and \ref{FactorSumOfWeights}, which look otherwise very abstract.
%%This continued fraction can be used to compute functions of matrices \cite{Giscard2011b}.
%%\begin{remark}[Combinatorial interpretation of continued fractions]
%%Theorem \ref{FactorSumOfWeights} extends results of \cite{Flajolet1980} and \cite{Flajolet2009} linking certain characteristic series of walks with continued fractions, thereby providing combinatorial interpretations to the continued fractions.
%%\end{remark}
%But before we give examples illustrating the Theorems above, we determine the depth at which the continued fraction terminates.


==> Graph_Proofs.tex <==
\section{Proofs for the Prime Factorisation on Graphs}
%In this section we prove the results presented in the preceding sections without proof. We begin by proving that $(W_\G,+,\odot)$ forms a noncommutative nonassociative near-algebra. We then prove the results of \S \ref{sec:WalkFactor} on the prime factorisation of walks.
%
%\subsection{The nesting near-algebra}\label{NONbilinear}
%For $(W_\G,+,\odot)$ to form a noncommutative nonassociative near $K$-algebra, we must verify that $(W_\G,+)$ is an abelian group, shown in \cite{Auslander1997}, and that the nesting product is compatible with the scalars and right distributive. 
%
%\textit{Compatibility with the scalars:} let $(k_1,\,k_2)\in K^2$, $a\in W_{\G;\,\alpha\omega}$ and $b\in W_{\G;\,\mu\mu}$. We show that $(k_1\,a)\odot (k_2\,b)=k_1k_2 (a\odot b)$.
%If $a\odot b=0$ the property is trivially true. Otherwise, 
%according to Definition \ref{def:Nesting}, $\exists!\, a_1\in W_{\G;\,\alpha\mu}$, $\exists!\, a_2\in W_{\G;\,\mu\omega}$ with $a\odot b= a_1\conc b\conc a_2$. Then $(k_1\,a)\odot (k_2\,b)= k_1 a_1\conc (k_2 b) \conc a_2$. Since concatenation is bilinear, $k_1 a_1\conc (k_2 b) \conc a_2=k_1k_2 \, (a_1\conc b\conc a_2)=k_1k_2 (a\odot b)$ and nesting is compatible with the scalars.
%
%\textit{Right-distributivity :} let $(a,b)\in W_{\G;\,\mu\mu}^2$ and $c\in W_{\G;\,\alpha\omega}$. We show that $c\odot(a+b)=c\odot a+c\odot b$. Walks $a$ and $b$ being cycles off the same vertex $\mu$ (otherwise $a+b=0$ and the property is trivially true), it follows that $c\odot a=0\iff c\odot b=0\iff c\odot (a+b)=0$ and the property is true as soon as $c\odot a$ or $b=0$. 
%Otherwise, definition \ref{def:Nesting} implies that $\exists!\, c_1\in W_{\G;\,\alpha\mu}$ and $\exists!\, c_2\in W_{\G;\, \mu\omega}$ such that $c\odot a= c_1\conc a\conc c_2$ and $c\odot b= c_1\conc b\conc c_2$. Since concatenation is bilinear we have
%$c\odot a+c\odot b= c_1\conc a\conc c_2+ c_1\conc b\conc c_2=c_1\conc (a+b)\conc c_2= c\odot (a+b)$ and nesting is right distributive.
%
%\textit{Failure of left-distributivity :} let $(a,b)\in W_{\G;\,\alpha\omega}^2$ and $c\in W_{\G;\,\mu\mu}$. We show that in general $(a+b)\odot c\neq a\odot c+b\odot c$. Suppose that both $a$ and $b$ visit $\mu$.  
%Then by Definition \ref{def:Nesting}, $\exists!\, a_1\in W_{\G;\,\alpha\mu}$ and $\exists!\, a_2\in W_{\G;\, \mu\omega}$ with $a\odot c = a_1\conc c\conc a_2$. Similarly, $b \odot c\neq0\Rightarrow\exists!\, b_1\in W_{\G;\,\alpha\mu}$ and $\exists!\, b_2\in W_{\G;\, \mu\omega}$ with $b\odot c = b_1\conc c\conc b_2$. Now $a\odot c+b\odot c =a_1\conc c\conc a_2+b_1\conc c\conc b_2\neq(a_1+b_1)\conc c\conc (a_2+b_2)=(a+b)\odot c$. 
%
%
%The nesting product is therefore compatible with the scalars and right-distributive with respect to $+$ but not left-distributive. It follows that $K\G_\odot=(W_\G,+,\odot)$ is a noncommutative nonassociative near $K$-algebra.
%

\subsection{Existence and uniqueness of the prime factorisation}\label{ExistsProof}



\subsection{Prime factorisations of $W_{\G;\,\alpha\omega}$ and $\Sigma_{\G;\,\alpha\omega}$}\label{SumProof}
\begin{remark}[Concatenating sets]
Let $A$ and $B$ be two sets of walks on $\G$. Then we write $A\conc B$ for the set obtained by concatenating every element of $B$ into every element of $A$.
\end{remark}

\noindent\tri We first prove Theorem \ref{FactorBasis}.

%\begin{remark}[Alternative proof]We may obtain Theorem \ref{FactorBasis} as a direct implementation of Algorithm \ref{AlgoCanFac} to sets of walks. Since the canonical factorisation of $w$ is obtained via the recursive use of Eqs.~(\ref{cycleSPLIT}) and (\ref{eq:FactorW}) and since this factorisation is unique, the set of walks $W_{\G;\,\nu_0\nu_p}$ is uniquely factorised through the recursive use of Eqs.~(\ref{WG}) and (\ref{AG}). We omit the details of this alternative approach.
%\end{remark} 
%





\vspace{1.5mm}\noindent\tri We prove Theorem \ref{FactorSum}.

\vspace{1.5mm}\noindent$\blacktriangleright$ We prove Theorem \ref{FactorSumOfWeights}.
\begin{proof}
This theorem follows from Theorem \ref{FactorSum} together with the properties of the weight function. %defined in Eq.~\eqref{eqn:Weightproperties}.
\end{proof}

%\subsection{The star-height of factorised walk sets}\label{StarHeightProof}


==> Introduction_Graph.tex <==
\section{Introduction}
\subsection{Context}
Walks on graphs are pervasive mathematical objects that appear in a wide range of fields from mathematics  and physics to engineering, biology and social sciences \cite{Godsil1993,Flajolet2009,Bollobas1998,Blanchard2011,Sheskin2010,Berg1993,Borgatti2009}.  Walks are perhaps most extensively studied in the context of random walks on lattices \cite{Lawler2010}, \sjt{where they are used to model} physical processes \cite{Burioni2005}. At the same time, it is difficult to find general `context-free' results concerning \sjt{walks: indeed, the properties of walks are almost always strongly dependent on the graph on which they take place.} For this reason, many results concerning walks on graphs are \sjt{intimately connected with} the specific context in which they appear.

Over the past 30 years, the \sjt{solutions} to a number of problems across many fields have been formulated in terms of sums of walks. Amongst the most important we must mention the early work by Brydges et al. in statistical physics \cite{Brydges1983} and the seminal work by Malioutov and coworkers \cite{Malioutov2006} concerning Gaussian belief \sjt{propagation in probabilistic graphical models. These previous works are unified by two underlying themes: firstly, that some quantities are most naturally expressed as sums of walks, and secondly, that these walk-sums can be reduced to more manageable expressions by resumming certain families of terms appearing in the sum. However, none of the existing studies address the question of how these resummations can be developed in a systematic fashion. Consequently, the results in the existing literature depend strongly on the context of their discovery, and are only applicable in a limited number of situations. The general feasibility of walk resummations for graphs of arbitrary structure thus remains an open problem. In this article we present a mathematically rigorous and general approach to the question of summing and resumming walks. In particular, we obtain an explicit expression for the sum of all walks between any two vertices of any weighted multi-digraph.}

\subsection{\sjt{A systematic approach to walk sums}}
\sjt{In this work we consider walks on (possibly weighted) directed graphs as mathematical entities in their own right.} 
We demonstrate that \sjt{these walks exhibit non-trivial properties that are largely \emph{independent} of the digraph on which they} take place. Foremost amongst these properties is \sjt{that any walk can be uniquely factorized into a product of prime walks, which we show are precisely the simple paths and simple cycles of the underlying graph.}\footnote{Simple paths and simple cycles are also known as self-avoiding walks and self-avoiding polygons, respectively.}. \sjt{An important consequence of this result is the existence of a universal closed-form expression} for the series of all walks between any two vertices of any finite (weighted) digraph: \sjt{namely,} a branched continued fraction of finite depth and breadth, which we provide. \sjt{This continued fraction} is the prime representation of the walk series, \sjt{an analog of the Euler product formulae} for the Riemann zeta function and other totally multiplicative functions in number theory. This universal continued fraction, which we present and prove here, has already found applications in the fields of matrix functions \cite{Giscard2011b}, differential calculus \cite{Giscard2014a}, quantum dynamics \cite{Giscard2014} and machine learning \cite{Giscard2014b}. Although seemingly disparate, many open questions in these disciplines are unified by their natural formulation in terms of sums of walks and thus benefit from the results presented here.

\sjt{The usual product operation} on the set $W_\G$ of all walks on a digraph $\G$ \sjt{is concatenation, which we denote here by $\conc$.}
%\textcolor{red}{Usually, the product operation between walks on graphs is the concatenation.
%set of all the walks on a digraph $\G$ is made into a $K$-algebra, known as the quiver
%algebra or path algebra $K\G$ \cite{Auslander1997}, by adjoining the operations of addition and
%concatenation to it. }
\sjt{Concatenation} is a very liberal operation: the concatenation $a\conc b$ of \sjt{two walks $a$ and $b$} is
non-zero whenever the final vertex of $a$ is the same as the initial vertex of $b$. This implies that both the
irreducible and the prime elements of the set of all walks equipped with the concatenation product, denoted $(W_\G,\conc)$, are the walks of \sjt{length 1 on $\G$: in other words, the edges} of $\G$.
Consequently, the factorisation of a walk $w$ on $\G$ into concatenations of prime walks is somewhat trivial. For this reason, we abandon the operation of concatenation and \sjt{define instead a new product between walks, which we term nesting and denote by $\odot$.} Nesting is a much more restrictive operation than concatenation, in that the nesting of two walks is non-zero only if the walks satisfy certain constraints.
As a result of these constraints, the \sjt{irreducible and prime elements of $(W_\G,\,\odot)$ are the simple paths and simple cycles of $\G$, rather than the edges of $\G$.} The rich structure that \sjt{the nesting operation induces} on walk sets is at the origin of the universal continued fraction formula for formal series of walks.
%Furthermore we prove that the factorisation of any walk into these prime elements always
%exists and is unique.
%Thanks to this result we obtain a novel representation for the set of walks on $\G$ and derive a %compact expression for the characteristic series of all the walks between any two vertices of $\G$.
%
%
% Of particular importance is the \emph{uniqueness} of the prime factorisation, a fact that was fully recognized during the $19$\tth century with the first examples of number fields where uniqueness does not hold.
%This observation gave rise to the notion of ideal, a concept of paramount importance in ring theory and abstract algebra \cite{Lang2002}. More recently, the study of unique factorisation and ideals was  extended to rings with zero divisors \cite{Galovich1978,Agargun1999}, noncommutative rings \cite{Cohn1963,Chatters1992,Lam2001} and nonassociative rings and algebras \cite{Brown1958,Zwier1971}.
%
%In this thesis we demonstrate that an equivalent to the fundamental theorem of arithmetic holds at the element level on the set of walks on any finite digraph equipped with a product operation we introduce, the nesting product. Thanks to this result, we obtain a continued fraction formulation for characteristic series of walks on such digraphs.



This article is organised as follows. In \S \ref{concepts}, we present the notation and terminology used throughout the article. In particular, we define the nesting product and establish its properties in  \S \ref{NestingDef}.
%In \ref{AlgebraDef} we define the nesting near-algebra $K\G_\odot$, the equivalent of the path algebra $K\G$ \cite{Auslander1997} with the concatenation replaced by the nesting product.
In \S \ref{sec:WalkFactor} we obtain \sjt{our central result: we prove the existence and uniqueness of the factorization of any walk on a digraph $\G$ into nesting products of primes (i.e.~the simple paths and simple cycles on $\G$).} We provide an \sjt{algorithm that produces} the prime factorisation of individual walks in \S\ref{Algosection} and a recursive formula to reduce sets of walks into nested sets of primes in \S\ref{SectionFactorBasis}. \sjt{In \S\ref{PathSumPrimeSeries} we exploit these results to present the prime representation of walk series.} \sjt{Specifically, we obtain in \S\ref{formal} an explicit branched continued fraction for the sum of all walks between any two vertices of any digraph, and in \S\ref{weightedsum} extend this result to the case of weighted digraphs.} Finally, the last section \S\ref{StarHeightsection} is devoted to \sjt{identifying the maximum} depth of this continued fraction.
%The results of this section are proven in sections \ref{ExistsProof}, \ref{AlgoVal} and \ref{SumProof}.
%%In \S\ref{StarHeightsection} we discuss the complexity of the prime factorisation of walks.
%Finally, in \S\ref{ExampleSection} we present examples illustrating our results.



%The fundamental theorem of arithmetic is arguably the most important result in the field of number theory \cite{Hardy1979}. It establishes the central role played by the prime numbers and has many profound consequences on the properties of integers. Of particular importance is the \emph{uniqueness} of the prime factorisation, a fact that was fully recognized during the $19$\tth century with the first examples of number fields where uniqueness does not hold.
%This observation gave rise to the notion of ideal, a concept of paramount importance in ring theory and abstract algebra \cite{Lang2002}. More recently, the study of unique factorisation and ideals was  extended to rings with zero divisors \cite{Galovich1978,Agargun1999}, noncommutative rings \cite{Cohn1963,Chatters1992,Lam2001} and nonassociative rings and algebras \cite{Brown1958,Zwier1971}.
%
%In this article we demonstrate that an equivalent to the fundamental theorem of arithmetic holds at the element level
%on the set of walks on any finite digraph equipped with a product operation we introduce, the nesting product. Thanks to this result, we obtain a continued fraction formulation for characteristic series of walks on such digraphs. This extends results of \cite{Flajolet1980} and \cite{Flajolet2009}. We give examples of applications of our results in combinatorics and language theory.











%
%Usually, the set of all the walks on a digraph $\G$ is made into a $K$-algebra, known as the quiver algebra or path algebra $K\G$ \cite{Auslander1997}, by adjoining the operations of addition and concatenation to it. Concatenation is a very liberal operation: the concatenation $a\conc b$\nomenclature{$\conc$}{Concatenation product} of two walks is non-zero whenever the final vertex of $a$ is the same as the initial vertex of $b$. This implies that both the irreducible and the prime elements of the path algebra are the walks of length 1, i.e.~the edges of $\G$. Consequently, the factorisation of a walk $w$ on $\G$ into concatenations of prime walks is somewhat trivial.
%%At the opposite, if one could uniquely factorise walks into less elementary prime walks we might obtain a novel and convenient way of representing and manipulating walks.
%For this reason, we abandon the operation of concatenation and introduce instead the nesting product as the product operation between walks on $\G$. Nesting is a much more restrictive operation than concatenation, in that the nesting of two walks is non-zero only if the walks satisfy certain constraints.
%As a result of these constraints, the irreducible and prime elements of the near-algebra obtained upon replacing the concatenation with the nesting product are the simple paths and simple cycles of $\G$, rather than its edges. Furthermore we prove that the factorisation of any walk into these prime elements always exists and is unique.
%Thanks to this result we obtain a novel representation for the set of walks on $\G$ and derive a compact expression for the sum of all the walks between any two vertices of $\G$ as a continued fraction involving only the simple paths and simple cycles of $\G$.
%
%This article is organised as follows. In \S \ref{concepts}, we present the notation and terminology used throughout the thesis. In \ref{NestingDef} we define the nesting product and establish its properties. In \ref{AlgebraDef} we define the nesting near-algebra $K\G_\odot$, the equivalent of the path algebra $K\G$ with the concatenation replaced by the nesting product. In \S \ref{sec:WalkFactor} we give the main results of the present thesis: (i) existence and uniqueness of the factorisation of any walk into nesting products of simple paths and simple cycles; (ii) an algorithm performing the factorisation; (iii) factorisation of walk sets as nested sets of simple paths and simple cycles; and (iv) factorisation of sums of walks and sums of weighted walks as finite continued fractions over the simple paths and simple cycles. The results of this section are proven in Appendices \ref{ExistsProof}, \ref{AlgoVal} and \ref{SumProof}. In \S \ref{ExampleSection} we present examples of the application of our results. Finally, in \S \ref{StarHeightsection} we discuss the complexity of the prime factorisation of walks. 

==> Required_Concepts_Graph.tex <==
\section{Required Concepts}\label{concepts}
\subsection{Notation and terminology}\label{NotationCh1}
A \emph{directed graph} or \emph{digraph} is a set of \emph{vertices} connected by \sjt{\emph{directed edges},} also known as arrows. An arrow $e$ starts at vertex $s(e)$ and terminates at vertex $t(e)$, which we write $e:\,s(e)\rightarrow t(e)$ or $(s(e)t(e))$.
Throughout this article, we let $\G=\big(\mc{V}(\G),\mc{E}(\G)\big)$ be a finite digraph with $\mc{V}(\mc{G})$ its vertex set and $\mc{E}(\mc{G})$ its edge set. This digraph may contain self-loops but not multiple edges, i.e.~we restrict ourselves to at most one directed edge from $\alpha\in\mc{V}(\G)$ to $\omega\in\mc{V}(\G)$. The latter restriction is solely for the purpose of notational clarity, and all of our results can be straightforwardly extended to cases where $\mc{G}$ contains multiple edges. We denote the vertices of $\G$ by numbers or Greek letters \sjt{$\alpha,\beta,\ldots$, as convenient.} The digraph obtained by deleting vertices $\alpha,\beta,\ldots$ and all edges incident on these vertices from $\G$ is written $\G\backslash\{\alpha,\beta,\ldots\}$.

A \emph{walk} $w$ of length $\ell(w)=n\ge1$ from $\mu_0$ to $\mu_{n}$ on $\G$ is a left-to-right sequence \sjt{$(\mu_0\mu_1),(\mu_1\mu_2),\cdots,(\mu_{n-1}\mu_n)$} of $n$ contiguous directed edges. This walk starts at $\mu_0$ and terminates at $\mu_n$
We \sjt{represent} $w$ by its vertex string $(\mu_0\,\mu_1\,\mu_2\,\cdots\,\mu_n)$ or by its vertex-edge sequence $(\mu_0)(\mu_0\mu_1)(\mu_1)\cdots\,(\mu_{n-1}\mu_n)(\mu_n)$.
If $\mu_0=\mu_n$, $w$ is termed a \textit{cycle} or closed walk; otherwise, $w$ is an open walk. When necessary, the initial vertex of $w$ will be denoted by $h(w)$, and the final vertex by $t(w)$.
The set of all walks on $\G$ is denoted by $W_{\G}$, and the set of all walks from vertex $\mu_0$ to vertex $\mu_n$ on $\G$ is denoted by $W_{\G;\,\mu_0\mu_n}$.

A \emph{simple path} is an open walk whose vertices are all distinct. The set of all the simple paths on $\G$ is denoted by $\Pi_{\G}$. The set of simple paths from $\alpha$ to $\omega$ is denoted by $\Pi_{\G;\,\alpha\omega}$. On any finite digraph $\G$, these sets are finite.

A \emph{simple cycle} is a cycle whose internal vertices are all distinct and different from the initial vertex. The set of all the simple cycles on $\G$ is denoted by $\Gamma_{\G}$, while the set of simple cycles off a specific vertex $\alpha$ is denoted by $\Gamma_{\G;\,\alpha}$. On any finite digraph $\G$, these sets are finite.

A \emph{trivial walk} is a walk of length 0 off any vertex $\mu \in \mathcal{V}(\G)$, denoted by $(\mu)$. \sjt{A trivial walk is a simple path, but not a simple cycle. Note that trivial walks are different from the \emph{empty walk}, denoted $0$, whose length is undefined.}

The \emph{concatenation} is a non-commutative product operation between walks. Let $w_1=(\alpha_1\cdots\alpha_\ell)\in W_\G$ and $w_2=(\beta_1\cdots\beta_{\ell'})\in W_\G$. Then the concatenation of $w_1$ with $w_2$ is defined as
\begin{equation}
w_1\conc w_2=
\begin{cases}
(\alpha_1\cdots\alpha_\ell\,\beta_2\cdots\beta_{\ell'}),&\textrm{if }\alpha_\ell\equiv \beta_1,\\
0,&\textrm{otherwise}.
\end{cases}
\end{equation}
The empty walk is absorbing for the concatenation, \sjt{i.e. for every $w\in W_{\G}$, we have $w\conc 0=0\conc w=0$.}
%
%Let $\mathfrak{V}=\{V\}$ be a collection of vector spaces, each of arbitrary finite dimension, such that $\mathfrak{V}$ is in one to one correspondence with the vertex set $\mc{V}(\G)$ of a finite directed graph $\G$. For simplicity we designate by $V_\mu\in\mathfrak{V}$ the vector space associated to vertex $\mu\in\mc{V}(\G)$. Let $\mathfrak{F}=\{\varphi_{\mu\to\nu}:V_\mu\to V_\nu\}$ be a collection of linear mappings in one to one correspondence with the edge set $\mc{E}(\G)$ of $\G$. We associate the linear mapping $\varphi_{\nu\ot\mu}\in\mathfrak{F}$ to the directed edge from $\mu$ to $\nu$.
%Then $\mathfrak{G}=(\mathfrak{V},\,\mathfrak{F})$ is a representation of the directed graph $\G$, which in this context is also called a \emph{quiver} \cite{Dersken2005,Savage2005}. The representation of a walk $w=(\alpha_1\alpha_2\cdots\alpha_\ell)\in W_\G$ is the linear mapping $\varphi_w$ obtained from the composition of the linear mappings representing the successive edges traversed by the walk $\varphi_w=\varphi_{\alpha_{\ell}\ot\alpha_{\ell-1}}\conc\cdots\conc\varphi_{\alpha_3\ot\alpha_2}\conc\varphi_{\alpha_{2}\ot\alpha_1}$. The representation of a trivial walk $(\mu)$ is the identity map $1_{\mu}$ on $V_\mu$ and the representation of the empty walk $0$ is the 0 map.
%
%\begin{remark}
%The utility of the quiver as a representation of a digraph is explained in Remark \ref{RepresentationLayers}, p. \pageref{RepresentationLayers}.
%\end{remark}



\subsection{The nesting product}\label{NestingDef}
We now turn to the definition and properties of the nesting product. Nesting is more restrictive than concatenation; in particular, \sjt{the nesting product of two walks is non-zero} only if they obey the following property:

\begin{definition}[Nestable property]\label{CanDef}
Consider $(a,b)\in W_{\G}^2$ with $b=\beta\,\beta_2\,\cdots\, \beta_q\, \beta$ a cycle off $\beta$, and $a=\alpha_1\,\alpha_2\,\cdots\beta\cdots\, \alpha_k$ a walk that visits $\beta$ at least once. \sjt{Let $\alpha_j=\beta$ be the first appearance of $\beta$ in $a$.} Then the couple $(a,b)$ is nestable if and only if one of the following conditions holds:
\begin{itemize}
\item[(i)] $a$ and $b$ are cycles off the same vertex $\beta$; or
\item[(ii)] \sjt{ $\{\alpha_1,\alpha_2,\ldots,\alpha_{j-1}\} \cap \{\beta_2,\ldots,\beta_q\} = \emptyset$. In other words, no vertex that $a$ visits before reaching $\beta$ for the first time is also visited by $b$.} 
\end{itemize}
\end{definition}

The nestable property describes the natural structure arising from the cycle-erasing  procedure \sjt{(also known as loop-erasing procedure) introduced by Lawler in \cite{Lawler1980,Lawler2010}. Consider traversing a walk $w$ on a graph, removing all simple cycles $c_i$ (where $1\leq i\leq n$) from $w$ in chronological order. Upon reaching the end of the walk, the surviving vertex string forms a simple path $p$. It can be seen that for any eliminated cycle $c$ whose head is on $p$, the couple $(p,c)$ is nestable.} \sjt{[Similarly, for any two eliminated cycles $c_i$ and $c_{j>i}$ that share at least one vertex, the couple $(c_i,c_j)$ is nestable. NB: not true!!] This provides a natural motivation for the nesting product as the inverse operation of the cycle-erasing procedure: the walk $w$ can be written as a nesting product involving the simple path $p$ and the erased simple cycles $c_1\cdots c_n$.}

\begin{definition}[Nesting product]\label{def:Nesting}
Let $(w_1,\,w_2)\in W_\G^2$ be two walks on $\G$. If the couple $(w_1,\,w_2)$ is not nestable, we define the nesting product to be $w_1\odot w_2=0$. Otherwise, let $w_1 = (\eta_1\,\eta_2\cdots \beta\cdots \eta_{\ell_1})$ be a walk of length $\ell_1$ and let $w_2 =(\beta\,\kappa_2\cdots\kappa_{\ell_2}\,\beta)$ be a cycle of length $\ell_2$ off $\beta$. Then the operation of nesting is defined by
\begin{subequations}
\begin{eqnarray}
\hspace{-5mm}\odot:~W_{\G}\times W_{\G}&\to& W_{\G},\\
(w_1,\,w_2)&\to&w_1\odot w_2=(\eta_1\,\eta_2\cdots\beta\,\kappa_2\cdots\kappa_{\ell_2}\,\beta\cdots \eta_{\ell_1}).
\end{eqnarray}
\end{subequations}
The walk $w_1\odot w_2$ of length $\ell_1+\ell_2$ is said to consist of $w_2$ nested into $w_1$. The vertex sequence of $w_1\odot w_2$ is formed by replacing the \emph{last} appearance of $\beta$ in $w_1$ by the entire vertex sequence of $w_2$.
\end{definition}


\begin{figure}[t!]
\begin{center}
\vspace{2mm}
\includegraphics[width=1 \textwidth]{NestingPicture.pdf}
\end{center}
\vspace{-2mm}
\caption[An example of nesting]{An example of nesting: the walk $w=\alpha_1\alpha_2\alpha_3\alpha_4\alpha_5\alpha_6\alpha_7\alpha_8\alpha_9\alpha_7\alpha_4$ is obtained upon inserting the triangle $c_1=\alpha_7\alpha_8\alpha_9\alpha_7$ into the square $c_2=\alpha_4\alpha_5\alpha_6\alpha_7\alpha_4$ and then into the simple path $p=\alpha_1\alpha_2\alpha_3\alpha_4$, that is $w=p\odot\big(c_2\odot c_1\big)$.}
\end{figure}

\noindent\tri Nesting is non-commutative and non-associative: for example, $11\odot131=1131$, while $131\odot11=1311$, and $\big(12\odot242\big)\odot11=11242$, while $12\odot\big(242\odot11\big)=0$.

\vspace{1.5mm}
\noindent\tri Nesting coincides with concatenation for cycles off the same vertex: \sjt{for $(c_1,c_2)\in W_{\G;\,\alpha\alpha}^2$ we have $c_1\odot c_2=c_1\conc c_2$. Consequently, nesting is associative over the cycles: if $c_3\in W_{\G;\,\alpha\alpha}$ then $(c_1\odot c_2)\odot c_3=c_1\odot (c_2\odot c_3)=c_1\odot c_2\odot c_3$. This in turn implies power-associativity over the cycles, so we can simply write $c^p$ for the nesting of a cycle $c$ with itself $p$ times, e.g. $1212121=121\odot121\odot121=121^3$. We interpret $c^0$ as the trivial walk off $h(c)$.}

\vspace{1.5mm}
\noindent\tri \sjt{Let $\mu\in\mathcal{V}(\G)$. Consider the trivial walk $(\mu)$ and observe that for any cycle $w\in W_{\G}$ visiting $\mu$ we have $(\mu)\odot w=w\odot (\mu)=w$. NB: not true!!} Therefore we say that a trivial walk is a local identity element on the cycles. For any open walk $w'\in W_{\G}$ visiting $\mu$, we have $w'\odot (\mu)=w'$ and we say that a trivial walk is a local right-identity element on the open walks.


\vspace{2mm}Finally, with the nesting product comes a notion of divisibility. This notion plays a fundamental role in the identification of irreducible and prime walks:
\begin{definition}[Divisibility]\label{def:divisibility}
Let $w$ and $w'$ be two walks. We say that $w'$ divides $w$, and write $w'\,|\,w$, if and only if $w$ can be written using non-zero nesting products involving $w'$.
A walk $w'$ that divides $w$ will be called a factor or divisor of $w$.
%
%$\exists\, (a,b)\in W_\G^2$ such that either $w=(a\odot w')\odot b$ or $w=a\odot (w'\odot b)$.
\end{definition}


\noindent This basic definition is equivalent to the following, more explicit formulation:
\begin{definition}
Let $w$ and $w'$ be two walks. Then we say that $w'$ divides
$w$, and write $w' \,|\,w$, if and only if one of the following conditions holds:
\begin{itemize}
\vspace{-1mm}
\item[(i)] there exists a walk $w''$ such that $w'|w''$ and $w''|w$; or
\item[(ii)] there exists $n\geq 0$ walks $w_1,\,w_2,\,\cdots,\, w_n$  and an integer $0\leq i\leq n$ such that $w=w_1\odot\cdots\odot w_i\odot w'\odot w_{i+1}\odot\cdots\odot w_n$.
\end{itemize}
\end{definition}

%
%
%\subsection{The nesting near-algebra}\label{AlgebraDef}
%Having established the properties of the nesting product, we now turn to determining the structure it induces on the sets of walks and their characteristic series. In order for the latter to be defined, we need to equip walk sets with an addition. To this end, and in the spirit of the path algebra $K\G$ \cite{Auslander1997}, we want to construct a $K$-algebra with the set of walks $W_\G$ as basis but equipped with the nesting product instead of the concatenation. However left-distributivity of the nesting product with respect to addition does not hold (\S \ref{NONbilinear}). Therefore, we define instead a near $K$-algebra equipped with the nesting product.
%
%\begin{definition}[Near $K$-algebra \cite{Auslander1997}]
%Let $K$ be an algebraic closed field and $A$ a set. Let $+$ and $\bullet$ be an addition and a product operation defined between elements of $A$, respectively. Then we say that $(A,+,\bullet)$ forms a near $K$-algebra if and only if $(A,+)$ is an abelian group, the $\bullet$ product is compatible with the elements of $K$ and right distributive with respect to $+$.
%\end{definition}
%
%
%\begin{definition}[Nesting near-algebra]
%Let $K$ be an algebraically closed field. The nesting near-algebra $K\G_\odot=(W_\G,\,+,\,\odot)$ is a near $K$-algebra. Its support set is the set of walks on $\G$ and with the product of two walks $w$, $w'$ given by the nesting product $w\odot w'$.
%%The addition of two walks $w$, $w'$ is non-zero if and only if $h(w)=h(w')$ and $t(w)=t(w')$.
%\end{definition}
%
%%\begin{remark}[Zero element]
%%The identity element with respect to addition in $K\G_\odot$ is denoted $0$ and is not to be confused with a trivial walk. This element is absorbing with respect to nesting, $w\odot 0=0\odot w =0,~\forall w\in W_\G$.
%%\end{remark}
%
%
%\begin{remark}[Three layers of representation]\label{RepresentationLayers}
%While we have defined an addition and a product operation between walks on digraphs, these operations can give rise to rather abstract objects. For example, let
%$w_1$ and $w_2$ be two walks with identical end points. Then, the object $w_{1,2}
%=w_1+w_2$ exists but seems rather difficult to comprehend.
%To resolve this difficulty, we use the notion of quiver, introduced in \S\ref{NotationCh1} and which facilitates the rigorous manipulation of sums and products of walks.
%For example, it is easier to understand $w_{1,2}$ as the object whose representation on the quiver $\mathfrak{V}$ is the linear map $\varphi_{w_{1,2}}=\varphi_{w_{1}}+\varphi_{w_{2}}$. In turn, the linear mappings of the quiver have representations in terms of matrices, which allow direct manipulation of sums, products and inverse of mappings. In the present study we therefore use these three layers: i) the basic layer is the near $K$-algebra $K\G_\odot$ and comprises the walks, their sums, products and we will see, their formal inverses; ii) these objects are then represented by linear mappings on the quiver, which constitutes our second layer; and finally iii) the third layer comprises the matrix representations of these mappings. Correspondences between these layers are given on Table \ref{LayerTable}.
%\end{remark}
%\begin{table}[t!]
%\begin{center}
%\renewcommand{\arraystretch}{1.3}
%\begin{tabular}{|m{1in}|m{1in}|m{1in}|}
%\hline \multicolumn{1}{|c|}{\textbf{Layer 1}}&\multicolumn{1}{c|}{\textbf{Layer 2}}&\multicolumn{1}{c|}{\textbf{Layer 3}}\\
%\hline
%\hline
%Near-algebra $K\G_\odot$ &Quiver $\mathfrak{V}$& Matrix space $\mathbb{C}^{n\times n}$    \\
%\hline
%Walk $w$ &Mapping $\varphi_w$ & Matrix $\matr{M}_{\varphi_w}$    \\
%\hline
%
%$w_{1+2}=w_1+w_2$ &$\varphi_{w_{1+2}}=\varphi_{w_1}+\varphi_{w_2}$ & $\matr{M}_{\varphi_{w_{1+2}}}=\matr{M}_{\varphi_{w_1}}+\matr{M}_{\varphi_{w_2}}$    \\
%\hline
%Concatenation\newline
%$w_{1\conc2}=w_1\conc w_2$ &Composition\newline $\varphi_{w_{1\conc 2}}=\varphi_{w_2}\conc\varphi_{w_1}$ & Multiplication\newline $\matr{M}_{\varphi_{w_{1\conc2}}}=\matr{M}_{\varphi_{w_2}}\,.\,\matr{M}_{\varphi_{w_1}}$    \\
%\hline
%Formal inverse\newline
%$w^{-1}$ &Composition inverse\newline$\varphi_{w^{-1}}=\varphi_{w}^{(-1)}$ & Matrix inverse\newline $\matr{M}_{\varphi_{w^{-1}}}=\matr{M}_{\varphi_{w}}^{-1}$    \\
%\hline
%\hline
%\end{tabular}
%\end{center}
%\vspace{-5mm}\caption{\label{LayerTable} Correspondences between the three layers of representation used in this article.}
%\end{table}
%

%\subsection{The nesting near-algebra}\label{AlgebraDef}
%In the spirit of the path algebra $K\G$\nomenclature{$K\G$}{Path algebra} \cite{Auslander1997}, we want to construct a $K$-algebra with the set of walks $W_\G$ as basis but equipped with the nesting product instead of the concatenation.
%However left-distributivity of the nesting product with respect to addition does not hold (\S \ref{NONbilinear}). We therefore define a near $K$-algebra equipped with the nesting product:
%
%\begin{definition}[Nesting near-algebra]
%From now on, we fix $K$ an algebraically closed field. The nesting near-algebra $K\G_\odot=(W_\G,\,+,\,\odot)$\nomenclature{$K\G_\odot$}{Nesting near-algebra} is the near $K$-algebra whose basis is the walks in $\G$ and with the product of two walks $w$, $w'$ given by the nesting product $w\odot w'$. The addition of two walks $w$, $w'$ is non-zero if and only if $h(w)=h(w')$ and $t(w)=t(w')$.
%\end{definition}
%
%%\begin{remark}[Zero element]
%%The identity element with respect to addition in $K\G_\odot$ is denoted $0$ and is not to be confused with a trivial walk. This element is absorbing with respect to nesting, $w\odot 0=0\odot w =0,~\forall w\in W_\G$.
%%\end{remark}
%
%The nesting near-algebra provides the algebraic structure necessary for an equivalent to the fundamental theorem of arithmetic to hold on digraphs.
%To progress, we now identify the irreducible and prime elements of $K\G_\odot$ induced by the nesting product. We recall that a walk $w\in K\G_\odot$ is irreducible if, whenever $\exists\, a\in W_\G$ with $a\,|\,w$, then either $a$ is trivial, or $a=w$ up to nesting with trivial walks (i.e. local identities). A walk $w\in K\G_\odot$ is prime if and only if $w\,|\,a\odot b\Rightarrow w\,|\,a$ or $w\,|\,b$.
%
%\begin{proposition}\label{irreducible}
%The set of irreducible walks is exactly $\Pi_\G\cup \Gamma_\G$. The irreducible walks are the prime elements of $K\G_\odot$.
%\end{proposition}
%\begin{remark}[Identifying the simple paths and simple cycles]
%The simple paths and simple cycles of the digraph $\G$ can be systematically obtained via the powers of its nilpotent adjacency matrix, see \cite{Staples2008, Schott2012}.\end{remark}
%We defer the proof of Proposition \ref{irreducible} to \S \ref{ExistsProof}. Having established the definition and properties of the nesting product as well as the irreducible and prime elements it induces in $K\G_\odot$, we turn to the factorisation of walks. 
